Cartesian closed bicategories: type theory and coherence

In this thesis I lift the Curry--Howard--Lambek correspondence between the simply-typed lambda calculus and cartesian closed categories to the bicategorical setting, then use the resulting type theory to prove a coherence result for cartesian closed bicategories. Cartesian closed bicategories---2-categories `up to isomorphism' equipped with similarly weak products and exponentials---arise in logic, categorical algebra, and game semantics. I show that there is at most one 2-cell between any parallel pair of 1-cells in the free cartesian closed bicategory on a set and hence---in terms of the difficulty of calculating---bring the data of cartesian closed bicategories down to the familiar level of cartesian closed categories. In fact, I prove this result in two ways. The first argument is closely related to Power's coherence theorem for bicategories with flexible bilimits. For the second, which is the central preoccupation of this thesis, the proof strategy has two parts: the construction of a type theory, and the proof that it satisfies a form of normalisation I call "local coherence". I synthesise the type theory from algebraic principles using a novel generalisation of the (multisorted) abstract clones of universal algebra, called "biclones". Using a bicategorical treatment of M. Fiore's categorical analysis of normalisation-by-evaluation, I then prove a normalisation result which entails the coherence theorem for cartesian closed bicategories. In contrast to previous coherence results for bicategories, the argument does not rely on the theory of rewriting or strictify using the Yoneda embedding. Along the way I prove bicategorical generalisations of a series of well-established category-theoretic results, present a notion of glueing of bicategories, and bicategorify the folklore result providing sufficient conditions for a glueing category to be cartesian closed.

==> biequivalence-langCartClosed-hirCartClosed.tex <==

We begin by extending the 2-categorical type theory $\hir$ with pseudo (bicategorical) cartesian closed structure. We take cartesian closed structure in the style of Hilken's 2-$\lambda$ calculus~\cite{Hilken1996} and but continue to employ Hirschowitz's notion of \Def{permutation equivalence} to handle constants.

The syntactic model for Hilken's type theory has strict products, constructed by context extension (\cf~also~\cite{Pitts2000}). However, his lax exponentials provide a natural template for the introduction of (lax or pseudo) products. Of course, one could opt to introduce cartesian closed structure in the style of $\langCartClosed$. We adopt Hilken's style---which requires significantly more introduction rules---because it is clear it models the structure we require, because it allows us to compare $\langCartClosed$ with the work of Hilken and Hirschowitz, and because we may in places employ lemmas from Hilken's or Hirschowitz's construction.

On terms, we have the standard constructions of simply-typed lambda calculus. To maintain consistency with $\langCartClosed$ we immediately introduce $n$-ary products for all $n$; this is clearly equivalent to the standard, binary, approach. Contexts and the grammar for types over a fixed 2-multigraph $\graph$ are exactly as in $\langCartClosed$. On rewrites, we introduce functorial operations of pairing, projection, lambda abstraction and application, with an invertible unit and counit for products and exponentials. 

Introduction rules for the type theory are collected together in Figures~\ref{fig:r:strict-ccc:terms} \&~\ref{fig:r:strict-ccc:rewrites}, where $\graph$ is a fixed 2-multigraph. We denote the corresponding type theory by $\hirCCC(\graph)$.

\input{rules/hir/ccc-intro-rules}

The fragment consisting only of judgements of the form $\Gamma \vdash t : B$ is then exactly the simply-typed lambda calculus; in particular, standard properties such as  weakening and permutation hold. Similarly, taking substitution on terms to be the usual meta-operation of capture-avoiding substitution, one obtains the standard substitution lemma; the only subtlety is that one must define $c(u_1, \dots, u_n)[v_j / y_j] := c(u_1[v_j / y_j], \dots, u_n[v_j / y_j])$ on constants. We collect these observations in the next lemma.

\begin{prooflesslemma}
For any 2-multigraph $\graph$, the following hold in $\hirCCC(\graph)$:
\begin{enumerate}
\item For any contexts $\Gamma := (x_i : A_i)_{i=1,\dots,n}$ and $\Delta$, and any context renaming $r : \Gamma \to \Delta$, the rule
\begin{center}
\binaryRule{\Gamma \vdash t : B}{r : \Gamma \to \Delta}{\Delta \vdash t[r(x_i) / x_i] : B}{}
\end{center}
is admissible.
\item The following rule is admissible:
\begin{prooftree}
\AxiomC{$x_1 : A_1, \dots, x_n : A_n \vdash t : B$}
\AxiomC{$(\Delta \vdash u_i : A_i)_{i=1,\dots, n}$}
\BinaryInfC{$\Delta \vdash t[u_i/x_i] : B$}
\end{prooftree} \qedhere
\end{enumerate}
\end{prooflesslemma}

Substitution on rewrites is defined using left whiskering and right whiskering. We extend the definition for $\hir$ with the following rules:
\begin{align*}
\seq{t_1, \dots, t_n}[\tau_i / x_i] &:= \seq{t_1[\tau_i / x_i], \dots, t_n[\tau_i / x_i]} \\
\pi_k(t)[\tau_i / x_i] &:= \pi_k\big(t[\tau_i / x_i]\big) \\
(\app{t}{u})[\tau_i / x_i] &:= \app{t[\tau_i / x_i]}{u[\tau_i / x_i]} \\
(\lam{x}{t})[\tau_i / x_i] &:= \lam{x}{t[\tau_i / x_i]} 
\end{align*}
where in the final rule we require that $x \notin \bigcup_i \fv(\tau_i)$. Similarly, for substitution of terms into rewrites we extend the definition for $\hir$ as follows:
\begin{align*}
\etaTimes{t}[u_i/x_i] &:= \etaTimes{t[u_i/x_i]} \\
\epsilonTimesInd{k}{t_1, \dots, t_n}[u_i/x_i] &:= \epsilonTimes{k}{t_1[u_i/x_i], \dots, t_n[u_i/x_i]} \\
\etaExp{t}[u_i/x_i] &:= \etaExp{t[u_i/x_i]} \\
\genEpsilonExp{x \bind t, u}[u_i / x_i] &:= \genEpsilonExp{x \bind t[u_i / x_i], u[u_i / x_i]} \qquad \text{ for } x \notin \bigcup_i \fv(u_i) \\
\seq{\tau_1, \dots, \tau_n}[u_i / x_i] &:= \seq{\tau_1[u_i / x_i], \dots, \tau_n[u_i / x_i]} \\
\pi_k(\tau)[u_i / x_i] &:= \pi_k(\tau[u_i / x_i]) \\
(\app{\tau}{\sigma})[u_i / x_i] &:= \app{\tau[u_i / x_i]}{\sigma[u_i / x_i]} \\
(\lam{x}{\tau})[u_i / x_i] &:= \lam{x}{\tau[u_i / x_i]} \qquad \text{ for } x \notin \bigcup_i \fv(u_i)
\end{align*}

On exponential structure this definition coincides with Hilken's. The weakening and substitution lemmas hold as for terms: the proofs are simple structural inductions.

\begin{prooflesslemma}
For any 2-multigraph $\graph$, the following rules are admissible in $\hirCCC(\graph)$:
\begin{center}
\binaryRule{x_1 : A_1, \dots, x_n : A_n \vdash t : B}{(\Delta \vdash \sigma_i : \rewrite{u_i}{u_i'} : A_i)_{i=1, \dots, n}}{\Delta \vdash t[\sigma_i / x_i] : \rewrite{t[u_i/x_i]}{t[u_i'/x_i]} : B}{}
\binaryRule{x_1 : A_1, \dots, x_n : A_n \vdash \tau : \rewrite{t}{t'} : B}{(\Delta \vdash u_i : A_i)_{i=1, \dots, n}}{\Delta \vdash \tau[u_i / x_i] : \rewrite{t[u_i/x_i]}{t'[u_i/x_i]} : B}{}
\end{center}
Moreover, for any contexts $\Gamma := (x_i : A_i)_{i=1,\dots,n}$ and $\Delta$ and context renaming $r : \Gamma \to \Delta$, the following rule is admissible:
\begin{center}
\binaryRule{\Gamma \vdash \tau : \rewrite{t}{t'} : B}
	{r : \Gamma \to \Delta}
	{\Delta \vdash \tau[r(x_i) / x_i] : \rewrite{t[r(x_i)  / x_i]}{t'[r(x_i)  / x_i]} : B}
	{} \vspace{-\treeskip}
\end{center}
\end{prooflesslemma}

We extend the equational theory $\equiv$ for $\hir(\graph)$ with rules governing the product and exponential structure: we specify functorality of each of the constructors, and naturality and triangle laws for each unit and counit. These rules are collected in Figures~\ref{fig:hir:functorality}--\ref{fig:hir:congruence-laws}. As for $\hir(\graph)$, the equational theory ensures that the following law is admissible:
\begin{center}
\binaryRule{x_1 : A_1, \dots, x_n : A_n \vdash \tau : \rewrite{t}{t'} : B}
	{(\Delta \vdash \sigma_i : \rewrite{u_i}{u_i'} : A_i)_{i=1, \dots, n}}
	{\Delta \vdash t'[\sigma_i / x_i] \vert \tau[u_i / x_i] \equiv \tau[u_i' / x_i] \vert t[\sigma_i / x_i] : \rewrite{t[u_i/x_i]}{t'[u_i'/x_i]} : B}
	{}
\end{center}
and so we obtain a substitution operation with signature
\begin{equation}\label{eq:substitution-typed}
\binaryRule{x_1 : A_1, \dots, x_n : A_n \vdash \tau : \rewrite{t}{t'} : B}
	{(\Delta \vdash \sigma_i : \rewrite{u_i}{u_i'} : A_i)_{i=1, \dots, n}}
	{\Delta \vdash \tau[\sigma_i / x_i] : \rewrite{t[u_i/x_i]}{t'[u_i'/x_i]} : B}
	{}
\end{equation}
by taking either of these two equivalent composites as the definition. This is the content of the following lemma.

\begin{mylemma} \todo{prove and fill in}
For any 2-multigraph $\graph$, the following rule is admissible in $\hir(\graph)$:
\begin{center}
\binaryRule{x_1 : A_1, \dots, x_n : A_n \vdash \tau : \rewrite{t}{t'} : B}
	{(\Delta \vdash \sigma_i : \rewrite{u_i}{u_i'} : A_i)_{i=1, \dots, n}}
	{\Delta \vdash t'[\sigma_i / x_i] \vert \tau[u_i / x_i] \equiv \tau[u_i' / x_i] \vert t[\sigma_i / x_i] : \rewrite{t[u_i/x_i]}{t'[u_i'/x_i]} : B}
	{}
\end{center}
\end{mylemma}

\input{rules/hir/ccc-eq-theory}

We claim that the syntactic model of $\hirCCC(\graph)$ is a 2-category equipped with bicategorical cartesian closed structure. This is established by the following sequence of lemmas. In each case it suffices to check the product structure; the results for exponentials follow as in Hilken's 2-$\lambda$ calculus~\cite{Hilken1996}.

\begin{mylemma}[Functorality of substitution] \label{lem:hir:ccc:funct}
For any 2-multigraph $\graph$ the following equalities hold in $\hirCCC(\graph)$. For derivable judgements $x_1 : A_1, \dots, x_n : A_n \vdash t : B$ and $(\Delta \vdash u_i : A_i)_{i=1,\dots,n}$:
\begin{enumerate}
\item \label{c:id-into-term} $t[\id_{u_i} / x_i] \equiv \id_{t[u_i/x_i]}$, 
\item \label{c:id-into-id} $\id_t[\id_{u_i} / x_i] \equiv \id_{t[u_i/x_i]}$,
\end{enumerate}
Moreover, for derivable judgements $x_1 : A_1, \dots, x_n : A_n \vdash \tau' \vert \tau : \rewrite{t}{t'} : B$ and $(\Delta \vdash \sigma_i' \vert \sigma_i : \rewrite{u_i}{u_i''} : A_i)_{i=1,\dots,n}$, 
\begin{enumerate}
\item[3.] \label{c:interchange} $(\tau' \vert \tau)[\sigma_i' \vert \sigma_i / x_i] \equiv \tau'[\sigma_i' / x_i] \vert \tau[\sigma_i / x_i]$
\end{enumerate}
\begin{proof}
Each proof is by structural induction on $t$. (\ref{c:id-into-term}) is straightforward, and we use it for the proof of (\ref{c:id-into-id}). For example, for projections we have
\begin{align*}
\id_{\pi_k(t)}[\id_{u_i} / x_i] &\overset{\text{def}}{\equiv} \pi_k(t)[\id_{u_i} / x_i] \vert \id_{\pi_k(t)}[u_i / x_i] \\
&\equiv \pi_k(t)[\id_{u_i} / x_i] \\ 
&\equiv \pi_k(t[\id_{u_i} / x_i]) \\
&\overset{(\ref{c:id-into-term})}{\equiv} \pi_k(\id_{t[u_i/x_i]}) \\
&\equiv \id_{\pi_k(t[u_i/x_i])}
\end{align*}
For (\ref{c:interchange}) the proof is identical to the one for $\hir(\graph)$. 
\end{proof}
\end{mylemma}

\begin{mylemma}[Clone laws] \label{lem:hir:ccc:clone-laws}
For any 2-multigraph $\graph$ following equalities hold in $\hirCCC(\graph)$. For derivable judgements $x_1 : A_1, \dots, x_n : A_n \vdash x_k : A_k$, $(\Delta \vdash \sigma_i : \rewrite{u_i}{u_i'} : A_i)_{i=1, \dots, n}$, and $x_1 : A_1, \dots, x_n : A_n \vdash \tau : \rewrite{t}{t'} : B$,
\begin{enumerate}
\item \label{c:rewrite-into-var-id} $\id_{x_k}[\sigma_i / x_i] \equiv \sigma_k$, 
\item \label{c:tau-with-vars} $\tau[x_i / x_i] \equiv \tau$, 
\item \label{c:tau-with-ids} $\tau[\id_{x_i} / x_i] \equiv \tau$, 
\end{enumerate}
Moreover, for derivable judgements \mbox{$x_1 : A_1, \dots, x_n : A_n \vdash \tau : \rewrite{t}{t'} : C$}, \\ \mbox{$(y_1 : B_1, \dots, y_m : B_m \vdash \sigma_i : \rewrite{u_i}{u_i'} : A_i)_{i=1, \dots, n}$} and \mbox{$(\Sigma \vdash \mu_j : \rewrite{v_j}{v_j'} : B_j)_{j=1,\dots,m}$},
\begin{enumerate}
\setcounter{enumi}{3}
\item \label{c:interchange-terms} $\tau[u_i / x_i][v_j / y_j] \equiv \tau\big[ u_i[v_j / y_j] / x_i \big]$
\item \label{c:interchange-rewrites} $t[\sigma_i/ x_i][\mu_j / y_j] \equiv t\big[ \sigma_i[\mu_j / y_j] / x_i \big]$,
\item \label{c:full-interchange} $\tau[\sigma_i / x_i][\mu_j / y_j] \equiv \tau\big[ \sigma_i[\mu_j / y_j] / x_i \big]$
\end{enumerate}
\begin{proof}
(\ref{c:rewrite-into-var-id}) follows just as for $\hir(\graph)$. Cases~(\ref{c:tau-with-vars}) and~(\ref{c:tau-with-ids}) are straightforward inductions. 

To prove~(\ref{c:full-interchange}) we use the two preceding cases--- each of which is proven by induction on the structure of the rewrite $\tau$---and a further induction on $\tau$. Indeed, by definition 
\begin{center}
$\tau[\sigma_i / x_i][\mu_j / y_j] \equiv t'[u_i' / x_i][\mu_j / y_j] \vert \tau[\sigma_i / x_i][v_j / y_j]$ 
$\tau\big[ \sigma_i[\mu_j / y_j] / x_i \big] \equiv t'\big[ \sigma_i[\mu_j / y_j] / x_i \big] \vert \tau\big[ u_i[v_j / y_j] / x_i \big]$.
\end{center}
Applying~(\ref{c:interchange-terms}) and~(\ref{c:interchange-rewrites}) to this second equality, we obtain 
\[\tau\big[ \sigma_i[\mu_j / y_j] / x_i \big] \equiv t'[\sigma_i / x_i][\mu_j / y_j] \vert \tau[u_i/x_i][v_j  / y_j]
\] 
Then we induct on the structure of $\tau$. For example, for $\etaTimes{}$ one obtains
\begin{small}
\begin{align*}
t'[u_i' / x_i][\mu_j / y_j] \vert \tau[\sigma_i / x_i][v_j / y_j] &\equiv \seq{\ind{\pi}(t)}[u_i'/x_i][\mu_j / y_j] \vert \etaTimes{t}[\sigma_i/x_i][v_j/y_j] \\
&\overset{\mathrm{def}}{\equiv} \seq{\ind{\pi}(t[u_i'/x_i][\mu_j / y_j])} \vert \big( \seq{\ind{\pi}(t)}[\sigma_i/ x_i] \vert \etaTimes{t}[u_i/x_i] \big)[v_j/y_j] \\
&\equiv \seq{\ind{\pi}\big(t[u_i'/x_i][\mu_j / y_j] \vert t[\sigma_i/ x_i][\mu_j / y_j]\big)} \vert \etaTimes{t[u_i/x_i][v_j/y_j]} \\
&\equiv \seq{\ind{\pi}(t[\sigma_i/x_i][\mu_j/v_j])} \vert \etaTimes{t[u_i/x_i][v_j/y_j]} \\
&\equiv t'[\sigma_i / x_i][\mu_j / y_j] \vert \tau[u_i/x_i][v_j  / y_j]
\end{align*}
\end{small}
as required. The other cases are similar.
\end{proof}
\end{mylemma}

Hence, we do indeed obtain a 2-category. 

\begin{mypropn}
For any 2-multigraph $\graph$, the following defines a 2-category we denote by $\hirCCCSyn(\graph)$. Objects are contexts $\Gamma, \Delta, \dots$. The 1-cells $\Gamma \to (y_j : B_j)_{j=1,\dots,m}$ are $m$-tuples of $\alpha$-equivalence classes of terms $(\Gamma \vdash t_j : B_j)_{j=1,\dots,m}$ derivable in $\hirCCC(\graph)$. The 2-cells are $\alpha{\equiv}$-classes of rewrites, with identities and vertical composition given pointwise by $\id_t$ and the $\vert$ operation. Horizontal composition is the substitution operation~(\ref{eq:substitution-typed}) and the identity on $\Gamma := (x_i : A_i)_{i=1,\dots,n}$ is $(\Gamma \vdash x_i : A_i)_{i=1,\dots,n}$.
\begin{proof}
The functorality of horizontal composition follows from Lemma~\ref{lem:hir:ccc:funct} and the three axioms from Lemma~\ref{lem:hir:ccc:clone-laws}.
\end{proof}
\end{mypropn}

The next step is to construct bicategorical cartesian closed structure on $\hirCCCSyn(\graph)$. We employ the same strategy as for $\langCartClosed(\graph)$: our starting point is reducing the problem to unary contexts.

\begin{mylemma}
For any 2-multigraph $\graph$, 
\begin{enumerate}
\item \label{c:context-to-unary-equivalence} For any context $\Gamma := (x_i : A_i)_{i=1,\dots, n}$ in $\hirCCC(\graph)$ there exists an adjoint equivalence \mbox{$\Gamma \leftrightarrows (p : \prodop_n(A_1, \dots, A_n))$} in $\hirCCCSyn(\graph)$,
\item \label{c:unary-products} For any unary contexts $(x : A)$ and $(x_1 : A_1), \dots, (x_n : A_n)$ there exists an adjoint equivalence of hom-categories
\begin{small}\begin{td}
\hirCCCSyn(\graph)\big( (x: X), (p : \prodop_n(A_1, \dots, A_n)\big) \arrow[bend left = 20]{r}{(\pi_1 \circ -, \dots, \pi_n \circ -)} \arrow[phantom]{r}[]{\adjUp} & 
\hirCCCSyn(\graph)\big( (x: X), (x_i : A_i)\big)) \arrow[bend left = 20]{l}{\seq{-, \dots, =}} 
\end{td}\end{small}
\end{enumerate}
\begin{proof}
For~(\ref{c:context-to-unary-equivalence}) we take maps $\Gamma \leftrightarrows (p : \prodop_n(A_1, \dots, A_n))$ given by $\Gamma \vdash \seq{x_1, \dots, x_n} : \prodop_n(A_1, \dots, A_n)$ and $\big( p : \prodop_n(A_1, \dots, A_n) \vdash \pi_i(p) : A_i \big)_{i=1,\dots, n}$. The unit and counit are given by $\etaTimes{p}$ and $(\epsilonTimesInd{1}{x_1, \dots, x_n}, \dots, \epsilonTimesInd{n}{x_1, \dots, x_n})$, respectively.

For~(\ref{c:unary-products}) the operations $\seq{-, \dots, =}$ and $\pi_k(-)$ are functorial by the rules of Figure~\ref{fig:hir:functorality}. The unit and counit are given by $\etaTimes{}$ and $(\epsilonTimesInd{1}{}, \dots, \epsilonTimesInd{n}{})$, respectively.
\end{proof}
\end{mylemma}

\begin{prooflesscor}
For any 2-multigraph $\graph$, the 2-category $\hirCCCSyn(\graph)$ has all finite products.
\end{prooflesscor}

Explicitly, the product structure on $\hirCCCSyn(\graph)$ is as follows. The $n$-ary product of contexts $(y_i^{(1)} : B_i^{(1)})_{i=1, \dots, m_1} \times \dots \times (y_i^{(1)} : B_i^{(n)})_{i=1, \dots, m_n}$ is the product of unary contexts \mbox{$(q_1 : \prodop_{m_1}(B_1^{(1)}, \dots, B_{m_1}^{(1)})) \times \dots \times (q_n : \prodop_{m_n}(B_1^{(n)}, \dots, B_{m_n}^{(n)}))$}. Then for \mbox{$\Gamma := (x_i : A_i)_{i=1,\dots, n}$} the projection $\pi_k : \Gamma \to A_k$ is the composite $\Gamma \xra{\simeq} (p : \prodop_n(A_1, \dots, A_n)) \xra{\pi_k} A_k$, \ie~the term $\Gamma \vdash \pi_k(\seq{x_1, \dots, x_n}) : A_k$. On the other hand, given contexts $\Delta_j := (y_i^{(j)} : B_i^{(j)})_{i=1,\dots,m_j}$ and maps $(\Gamma \to \Delta_j)_{j=1,\dots,n}$ given by terms $(\Gamma \vdash t_i^{(j)} : B_i^{(j)})_{i=1, \dots, m_j}$ for $j = 1, \dots, n$, the $n$-ary pairing $\Gamma \to \prod_{j=1}^n \Delta_j$ is the $n$-ary pairing of the composite 
\[
\Gamma \to \Delta_j \xra{\simeq} (q_j : \prodop_{m_j}(B_1^{(j)}, \dot, B_{m_j}^{(j)}))
\]
which is the term $\Gamma \vdash \seq{t_1^{(j)}, \dots, t_{m_j}^{(j)}} : \prodop_{m_j}(B_1^{(j)}, \dots, B_{m_j}^{(j)})$. Thus, the $n$-ary pairing is the term
\[
\Gamma \vdash \seq{\seq{t_1^{(1)}, \dots, t_{m_1}^{(1)}}, \dots, \seq{t_n^{(n)}, \dots, t_{m_n}^{(n)}}} : \prodop_n (\prod_{j=1}^{m_1} B_j^{(1)}, \dots, \prod_{j=1}^{m_n} B_j^{(n)})
\]
In particular, given $\widebar{u} := (x : X \vdash u : \exptype{A}{B})$, the map $\widebar{u} \times (a : A) : (x : X) \times (a : A) \to (f: \exptype{A}{B}) \times (a : A)$ is 
\begin{align*}
\widebar{u} \times (a : A) &= \seq{\widebar{u} \circ \pi_1, \pi_2} \\	
&= \seq{(x : X, a : A \vdash u[\pi_1\seq{x,y} / x] : \exptype{A}{B}), (x : X, a : A \vdash \pi_2\seq{x, y} : A)}) \\
&= \big( (x : X, a : A \vdash \pi_1(p) : \exptype{A}{B}), (x : X, a : A \vdash \pi_2(p) : A) \big) 
\end{align*}
where $p := \seq{u[\pi_1\seq{x,y} / x], \pi_2(\seq{x, y})}$.

We now turn to constructing exponentials in $\hirCCCSyn(\graph)$. We define the evaluation map $\eval_{A,B} : (f : \exptype{A}{B}) \times (a : A) \to (b : B)$ to be given by application, as the term $(f : \exptype{A}{B}, a : A \vdash \app{f}{a} : B)$, so that---taking $\widebar{u}$ as defined above---$\eval_{A,B} \circ (\widebar{u} \times (a : B))$ is the following term (\cf~Equation~\ref{eq:eval-circ-u-times-a-pseudo}):
\begin{equation} 
x : X, a : A \vdash \app{\pi_1(\seq{u[\pi_1\seq{x,y} / x], \pi_2(\seq{x, y})})}{\pi_2(\seq{u[\pi_1\seq{x,y} / x], \pi_2(\seq{x, y})})} : B
\end{equation}
As in $\langCartClosed$, the adjoint equivalence we require arises from the unit and counit $\etaExp{}$ and $\genEpsilonExp{}$, modulo rewrites to reduce terms such as $\pi_1\seq{x,y}$ to variables.

\begin{mylemma}
For any 2-multigraph $\graph$, there exists an adjoint equivalence
\begin{small}\begin{td}
\hirCCCSyn(\graph)\big( (x: X), (f : \exptype{A}{B}) \big) \arrow[bend left = 20]{r}{\eval \circ (- \times (a : A)) } \arrow[phantom]{r}[]{\adjUp} & 
\prod_{i=1}^n \hirCCCSyn(\graph)\big( (x: X, a : A), (b : B)\big)) \arrow[bend left = 20]{l}{\lambda} 
\end{td}\end{small}
in $\hirCCCSyn(\graph)$.
\begin{proof}
We define $\lambda(x : X, a : A \vdash t : B) := ( x: X \vdash \lam{a}{t} : \exptype{A}{B})$. This is functorial by the rules of Figure~\ref{fig:hir:functorality}. It remains to define the unit and counit; the definition is analogous to that for $\langCartClosed$. Indeed, we begin by defining a pair of invertible rewrites $\tau_1, \tau_2$ by
\begin{gather*}
\tau_1 := \pi_1(\seq{u[\pi_1\seq{x,y} / x], \pi_2(\seq{x, y})}) \XRA{\epsilonTimesInd{1}{}} u[\pi_1\seq{x,y} / x] \XRA{u[\epsilonTimesInd{1}{} / x]} u[x/x] = u \\
\tau_2 := \pi_2(\seq{u[\pi_1\seq{x,y} / x], \pi_2(\seq{x, y})}) \XRA{\epsilonTimesInd{2}{}} \pi_2(\seq{x, y}) \XRA{\epsilonTimesInd{2}{}} y
\end{gather*}
so that we may define the unit $\etaExp{u}$ as the composite
\begin{small}
\[
u \XRA{\etaExp{u}} \lam{a}{(\app{u}{a})} \XRA{\lam{a}{(\app{\tau_1^{-1}}{\tau_2^{-1}})}} \lam{a}{\app{\big(\pi_1(\seq{(\lam{a}{t})[\pi_1\seq{x,y} / x], \pi_2(\seq{x, y})})\big)}{\big(\pi_2(\seq{u[\pi_1\seq{x,y} / x], \pi_2(\seq{x, y})})\big)}}
\]
\end{small}
and the counit $\epsilonExp_{t}$ similarly as the composite
\begin{small}
\[
\app{\big(\pi_1(\seq{(\lam{a}{t})[\pi_1\seq{x,y} / x], \pi_2(\seq{x, y})})\big)}{\big(\pi_2(\seq{(\lam{a}{t})[\pi_1\seq{x,y} / x], \pi_2(\seq{x, y})})\big)} \XRA{\app{\tau_1}{\tau_2}} \app{(\lam{a}{t})}{a} \XRA{\genEpsilonExp{a \bind t, a}} t
\]
\end{small}
The triangle laws hold by naturality of each of the defining components and the triangle laws of Figure~\ref{r:hir:triangleLaws}. Since $\etaExp{}$ and $\epsilonExp$ are clearly invertible, we obtain the required adjoint equivalence. 
\end{proof}
\end{mylemma}

\begin{prooflesscor}
For any 2-multigraph $\graph$ the syntactic model $\hirCCCSyn(\graph)$ is a 2-category with bicategorical cartesian closed structure.
\end{prooflesscor}

\subsection{Constructing the equivalence}

\subsubsection{Defining the pseudofunctors} \label{sec:ccc:biequivalence-pseudofunctors}

We begin by constructing pseudofunctors $\into{-} : \hirCCCSyn(\graph) \leftrightarrows \termCatCCC(\graph) : \out{({-})}$ between the respective syntactic models. As with biclones, the first step is constructing suitable maps on terms. The maps extend the maps $\into{-}$ and $\out{({-})}$ for biclones in the natural way.

%\begin{mydefn}
%For any 2-multigraph $\graph$ we define the \Def{terms} in $\langCartClosed(graph)$ as be expressions generated by the grammar extending that for terms in $\langBiclone(\graph)$ as follows
%\begin{small}
%\[
%t, u_1, \dots, u_n ::= \dots \st \pi_k(x) \st \pair{u_1, \dots, u_n} \st \evalterm(x,y) \st \lam{x}{t}
%\]
%\end{small}
%and the \Def{rewrites} to be expressions generated by the grammar extending that for $\langBiclone(\graph)$ with the rules
%\[
%\tau, \sigma, \sigma_1, \dots, \sigma_n ::= \dots \st \epsilonTimesInd{k}{} \text{  } (k \in \Nat) \st \transTimes{\sigma_1, \dots, \sigma_n} \st \epsilonExpRewr{} \st \transExp{x \bind \tau} 
%\]
%Similarly we define the \Def{terms} and \Def{rewrites} in $\hirCCC(\graph)$ to be expressions generated by the grammar formed by extending that for $\hir(\graph)$ with the rules
%\begin{align*}
%t, u, u_1, \dots, u_n &::= \dots \st \pi_k(t) \st \seq{u_1, \dots, u_n} \st \app{t}{u} \st \lam{x}{t}  \\
%\tau, \sigma, \sigma_1, \dots, \sigma_n &::= \dots \st \etaTimes{} \st \epsilonTimesInd{k}{} \text{  } (k \in \Nat) \st \etaExp{} \st \epsilonExp \st \pi_k(\tau) \st \seq{\sigma_1, \dots, \sigma_n} \st \app{\tau}{\sigma} \st \lam{x}{\tau} 
%\qedhere
%\end{align*}
%\end{mydefn}

We then extend the definitions of the mappings $\out{({-})} : \langBiclone(\graph) \leftrightarrows \hir(\graph) : \into{-}$ to mappings $\out{({-})} : \langCartClosed(\graph) \leftrightarrows \hirCCC(\graph) : \into{-}$. Here we need to translate between the universal-arrows and unit-counit formulations of bicategorical cartesian closed structure. The following lemma relates the two perspectives.

\begin{mylemma}
For any 2-multigraph $\graph$, the following equalities are derivable in $\langCartClosed(\graph)$:
\begin{center}
\binaryRule	{\Gamma \vdash u : \prodop_n(A_1, \dots, A_n)}
		{(\Gamma \vdash \alpha_i : \rewrite{\hcomp{\pi_i}{u}}{t_i} : A_i)_{i=1, \dots, n}}
		{\Gamma \vdash \transTimes{\alpha_1, \dots, \alpha_n} \equiv \pair{\alpha_1, \dots, \alpha_n} \vert \etaTimes{u} : \rewrite{u}{\pair{t_1, \dots, t_n}} : \prodop_n(A_1, \dots, A_n)}
		{}

\begin{bprooftree} 
\AxiomC{$\Gamma, x : A \vdash t : B$ \:\quad\: $\Gamma \vdash u : \exptype{A}{B}$} 
\noLine 
\UnaryInfC{$\Gamma, x : A \vdash \alpha : \rewrite{\genevalterm{\wkn{u}{x}, x}}{t} : B$}  
\UnaryInfC{$\Gamma \vdash \transExp{x \bind \alpha} \equiv (\lam{x}{\alpha}) \vert \etaExp{u}  : \rewrite{u}{\lam{x}{t}} : \exptype{A}{B}$} 
\end{bprooftree} 
\end{center}
\begin{proof}
Follows from the respective universal properties of $\transTimes{\alpha_1, \dots, \alpha_n}$ and $\transExp{x \bind \alpha}$.
\end{proof}
\end{mylemma}

The translation is then the natural one.

\begin{myconstr} \label{constr:cart-closed-out}
For any 2-multigraph $\graph$, define a mapping from terms in $\langCartClosed(\graph)$ to terms in $\hirCCC(\graph)$ by extending the mapping $\out{({-})}$ for $\langBiclone(\graph)$ as follows: 
\begin{align*}
\begin{aligned}[c]
\out{\pi_k(p)} &:= \pi_k(p) \\
\out{\evalterm(f,a)} &:= \app{f}{a}
\end{aligned}
\qquad\qquad\qquad
\begin{aligned}[c]
\out{\pair{t_1, \dots, t_n}} &:= \seq{\out{t_1}, \dots, \out{t_n}} \\
\out{\lam{x}{t}} &:= \lam{x}{\out{t}}
\end{aligned}
\end{align*} 
Further extend the map on rewrites in $\langBiclone(\graph)$ as follows:
\begin{align*}
\begin{aligned}[c]
\out{\epsilonTimesInd{k}{t_1, \dots, t_n}} &:= \epsilonTimesInd{k}{\out{t_1}, \dots, \out{t_n}} \\
\out{\transTimes{\sigma_1, \dots, \sigma_n}} &:= \seq{\out{\sigma_1}, \dots, \out{\sigma_n}} \vert \etaTimes{\out{u}} 
\end{aligned}
\qquad\qquad\qquad
\begin{aligned}[c]
\out{\epsilonExpRewr{t}} &:= \genEpsilonExp{x \bind \out{t}, x} \\
\out{\transExp{x \bind \tau}} &:= (\lam{x}{\out{\tau}}) \vert \etaTimes{\out{u}}
\end{aligned}
\end{align*}
\qedhere
\end{myconstr}

The construction is the same as the biclone case. It is elementary to check this definition respects $\alpha$-equivalence and the equational theory~$\equiv$.

\begin{prooflesslemma} \todo{check this carefully!}
For any 2-multigraph $\graph$,
\begin{enumerate}
\item For all derivable terms $t, t'$ in $\langCartClosed(\graph)$, if $t \aeq t'$ then $\out{t} \aeq \out{t'}$, 
\item For all derivable rewrites $\tau, \tau'$ in $\langCartClosed(\graph)$, if $\tau \aeq \tau'$ then $\out{\tau} \aeq \out{\tau}$, 
\item If $\Gamma \vdash t : B$ in $\langCartClosed(\graph)$ then $\Gamma \vdash \out{t} : B$ in $\hirCCC(\graph)$, 
\item If $\Gamma \vdash \tau : \rewrite{t}{t'} : B$ in $\langCartClosed(\graph)$ then $\Gamma \vdash \out{\tau} : \rewrite{\out{t}}{\out{t'}} : B$ in $\hirCCC(\graph)$,
\item If $\Gamma \vdash \tau \equiv \tau' : \rewrite{t}{t'} : B$ in $\langCartClosed(\graph)$ then $\Gamma \vdash \out{\tau} \equiv \out{\tau'} : \rewrite{\out{t}}{\out{t'}} : B$ in $\hirCCC(\graph)$. \qedhere
\end{enumerate}
\end{prooflesslemma}

Hence the mapping $\out{({-})}$ lifts to a map on hom-categories $\termCatCCC(\graph)(\Gamma, \Delta) \to \hirCCCSyn(\graph)(\Gamma, \Delta)$; setting $\out{\Gamma} := \Gamma$ for all contexts $\Gamma$, one obtains a strict pseudofunctor.

\begin{mypropn}
The mapping $\out{({-})}$ extends to a strict pseudofunctor \mbox{$\termCatCCC(\graph) \to \hirCCCSyn(\graph)$}. 
\begin{proof}
Exactly as in Proposition~\ref{prop:out-is-a-pseudofunctor}.
\end{proof}
\end{mypropn}

We think of $\out{({-})}$ as a \emph{strictification} of $\termCatCCC(\graph)$. In particular, the canonical 2-cells $\postName$ and $\pushName$ are sent to the identity.

\begin{mylemma} \label{lem:out-push-post-id} \quad
\begin{enumerate}
\item For any derivable judgements $(\context \vdash t_j : B_j)_{j=1, \dots, m}$ and $\subContext$ in $\langCartClosed(\graph)$, the judgement
\begin{small}
\[
\Delta \vdash \out{\post{t; \ind{u}}} \equiv \id_{\seq{\out{\ind{t}}}[\out{u_i}/x_i]} : \rewrite{\seq{\out{t_1}, \dots, \out{t_m}}[\out{u_i}/x_i]}{\seq{\out{t_1}, \dots, \out{t_m}}[\out{u_i}/x_i]} : \prodop_m(B_1, \dots, B_m)
\]
\end{small}
is derivable in $\hirCCC(\graph)$,
\item For any derivable judgements $\context, x : A \vdash t : B$ and $\subContext$ in $\langCartClosed(\graph)$, the judgement
\[
\Delta \vdash \out{\push{t}{\ind{u}}} \equiv \id_{(\lam{x}{\out{t})}[\out{u_i}/x_i]} : \rewrite{(\lam{x}{\out{t})}[\out{u_i}/x_i]}{(\lam{x}{\out{t})}[\out{u_i}/x_i]} : \exptype{A}{B}
\] 
is derivable in $\hirCCC(\graph)$.
\end{enumerate}
\begin{proof}
By definition $\post{t; \ind{u}} = \transTimes{\tau_1, \dots, \tau_k}$ for 
\[
\tau_k := \hpi{k}{\hcomp{\pair{t_1, \dots, t_m}}{\ind{u}}} \XRA{\assoc{}^{-1}} \hcompthree{\pi_k}{\pair{t_1, \dots, t_m}}{\ind{u}} \XRA{\hcomp{\epsilonTimesInd{k}{}}{\ind{u}}} \hcomp{t_k}{\ind{u}}
\]
so 
\begin{align*}
\out{\post{t; \ind{u}}} &= \seq{\out{\tau_1}, \dots, \out{\tau_m}} \vert \etaTimes{\out{\hcomp{\pair{t_1, \dots, t_m}}{\ind{u}}}} \\
	&\equiv \seq{\epsilonTimesInd{1}{\ind{\out{t}[\out{u_i}/x_i]}}, \dots, \epsilonTimesInd{m}{\ind{\out{t}[\out{u_i}/x_i]}}} \vert \etaTimes{\seq{\out{t_1}[\out{u_i}/x_i], \dots, \out{t_m}[\out{u_i}/x_i]}} \\
	&\equiv \id_{\seq{\out{t_1}[\out{u_i}/x_i], \dots, \out{t_m}[\out{u_i}/x_i]}}
\end{align*}
by the triangle laws. The argument for $\pushName$ is similar.
\end{proof}
\end{mylemma}

To extend the map $\into{-}$ to cartesian closed structure we need to take account of the variable binding. We therefore define it in stages. Our first step is taking the natural definition on terms.

\begin{myconstr} \label{constr:ccc:into-terms}
For any 2-multigraph $\graph$, define a mapping from terms in $\hirCCC(\graph)$ to terms in $\langCartClosed(\graph)$ by extending the definition for $\hir(\graph)$ as follows:
\begin{align*}
\begin{aligned}[c]
\into{\pi_k(t)} &:= \hcomp{\pi_k}{\into{t}} \\
\into{\seq{t_1, \dots, t_n}} &:= \pair{\into{t_1}, \dots, \into{t_n}} 
\end{aligned}
\qquad\qquad\qquad
\begin{aligned}[c]
\into{\app{t}{u}} &:= \hcomp{\evalterm}{\into{t}, \into{u}} \\
\into{\lam{x}{t}} &:= \lam{x}{\into{t}}
\end{aligned}
\end{align*} 
\end{myconstr}

This mapping respects typing and $\alpha$-equivalence. 

\begin{prooflesslemma} \todo{check this carefully!}
For any 2-multigraph $\graph$,
\begin{enumerate}
\item For all derivable terms $t, t'$ in $\hirCCC(\graph)$, if $t \aeq t'$ then $\into{t} \aeq \into{t'}$, 
\item If $\Gamma \vdash t : B$ in $\hirCCC(\graph)$ then $\Gamma \vdash \into{t} : B$ in $\langCartClosed(\graph)$. \qedhere
\end{enumerate}
\end{prooflesslemma}

To extend this definition to rewrites we would like some means of reducing explicit substitutions to capture-avoiding substitutions. For example, in $\hirCCC(\graph)$ the $\beta$-reduction rewrite $\genEpsilonExp{x \bind t, u}$ in context $\Gamma$ has type $\app{(\lam{x}{t})}{u} \To t[u/x]$. Taking the obvious $\beta$-reduction rewrite in $\langCartClosed(\graph)$ only yields a rewrite $\hcomp{\evalterm}{\lam{x}{\into{t}}, \into{u}} \To \hcomp{\into{t}}{\id_\Gamma, x \mapsto \into{u}}$. Similarly, in $\hirCCC(\graph)$ the unit of the exponential has type $t \To \lam{x}{(\app{t}{x})}$. This becomes $\into{t} \To \into{\lam{x}{\app{t}{x}}} = \lam{x}{\heval{\into{t}, x}}$ in $\langCartClosed(\graph)$, but $\etaExp{\into{t}}$ has type $\into{t} \To \lam{x}{\heval{\wkn{\into{t}}{x}, x}}$. To deal with both these cases we make use of an auxiliary rewrite $\sub{t}{u_1, \dots, u_n} : \hcomp{\into{t}}{x_i \mapsto \into{u_i}} \To \into{t[u_i/x_i]}$; as in the biclone case, this will also make up part of the data of the pseudofunctor $\hirCCCSyn(\graph) \to \termCatCCC(\graph)$. 

In contrast with the $\langBiclone$ case, the fact that lambda abstraction binds a variable means we must first define $\subName$ on weakenings (more generally, on context renamings). This is analogous to the simply-typed lambda calculus, where one usually proves lemmas about weakening as a means of proving lemmas about substitution (for example, in the case of the usual Substitution Lemma).  We call this 2-cell $\contName$ for \emph{context renaming}.

\begin{myconstr}
For any 2-multigraph $\graph$ and context renaming $r$ we construct a rewrite $\cont{t}{r}$ so that the rule
\begin{center}
\binaryRule{\Gamma \vdash \into{t} : B}{r : \Gamma \to \Delta}{\Delta \vdash \cont{t}{r} : \rewrite{\hcomp{\into{t}}{x_i \mapsto r(x_i)}}{\into{t[r(x_i)/x_i]}} : B}{}
\end{center}
is admissible by induction on the derivation of $t$ as follows:
\begin{small}
\begin{gather*}
\cont{x_k}{\ind{u}} := \hcomp{x_k}{x_i \mapsto \into{u_i}} \XRA{\indproj{k}{}} \into{u_k} \\
\cont{c(\ind{u})}{\ind{v}} := \hcompthree{c}{\into{u_1}, \dots, \into{u_n}}{\into{\ind{v}}} \XRA{\assoc{}} \hcomp{c}{\hcomp{\into{\ind{u}}}{\into{\ind{v}}}} \XRA{\hcomp{c}{\contName, \dots, \contName}} \hcomp{c}{\into{\ind{u}[v_j/y_j]}} \\
\cont{\pi_k(t)}{\ind{u}} := \hcomp{\hpi{k}{\into{t}}}{\into{u_i}} \XRA{\assoc{}} \hpi{k}{\hcomp{\into{t}}{\into{u_i}}} \XRA{\hpi{k}{\contName}} \hpi{k}{\into{t[u_i/x_i]}} \\
\cont{\seq{t_1, \dots, t_n}}{\ind{u}} := \hcomp{\pair{\into{t_1}, \dots, \into{t_n}}}{\into{u_i}} \XRA{\postName } \pair{\hcomp{\into{\ind{t}}}{\into{u_i}}} \XRA{\pair{\contName, \dots, \contName}} \pair{\into{\ind{t}[u_i/x_i]}} \end{gather*}
\end{small}
and 
\begin{small}
\begin{align*}
\cont{\app{t}{u}}{\ind{v}} := \hcomp{\heval{\into{t}, \into{u}}}{\into{\ind{v}}} &\XRA{\assoc{}} \heval{\hcomp{\into{t}}{\into{\ind{v}}}, \hcomp{\into{u}}{\into{\ind{v}}}} \\ 
		&\XRA{\heval{\contName, \contName}} \heval{\into{t[v_j/y_j]}}, {\into{u[v_j/y_j]}}  \\[8pt]
\cont{\lam{x}{t}}{\ind{u}} := \hcomp{\lam{x}{\into{t}}}{\into{\ind{v}}} &\XRA{\pushName} \lam{x}{\hcomp{\into{t}}{x, \wkn{\into{u}}{x}}} \\ 
		&\XRA{\lam{x}{\hcomp{\into{t}}{x, \cont{u}{\mathrm{inc}_x}}}} \lam{x}{\hcomp{\into{t}}{x, \into{u}}} \\ 					&\XRA{\lam{x}{\contName}} \lam{x}{\into{t[x / x, u_i/x_i]}}
\end{align*}
\end{small}
\end{myconstr}

We can now define $\subName$. The construction is identical, except that we make use of $\contName$ for the lambda abstraction case.

\begin{myconstr}
For any 2-multigraph $\graph$ we construct a rewrite $\sub{t}{\ind{u}}$ so that the rule
\begin{center}
\binaryRule{x_1 : A_1, \dots, x_n : A_n \vdash \into{t} : B}{(\Delta \vdash \into{u_i} : A_i)_{i=1,\dots, n}}{\Delta \vdash \sub{t}{\ind{u}} : \rewrite{\hcomp{\into{t}}{x_i \mapsto \into{u_i}}}{\into{t[u_i/x_i]}} : B}{}
\end{center}
is admissible by induction on the derivation of $t$ as follows:
\begin{small}
\begin{gather*}
\sub{x_k}{\ind{u}} := \hcomp{x_k}{x_i \mapsto \into{u_i}} \XRA{\indproj{k}{}} \into{u_k} \\
\sub{c(\ind{u})}{\ind{v}} := \hcompthree{c}{\into{u_1}, \dots, \into{u_n}}{\into{\ind{v}}} \XRA{\assoc{}} \hcomp{c}{\hcomp{\into{\ind{u}}}{\into{\ind{v}}}} \XRA{\hcomp{c}{\subName, \dots, \subName}} \hcomp{c}{\into{\ind{u}[v_j/y_j]}} \\
\sub{\pi_k(t)}{\ind{u}} := \hcomp{\hpi{k}{\into{t}}}{\into{u_i}} \XRA{\assoc{}} \hpi{k}{\hcomp{\into{t}}{\into{u_i}}} \XRA{\hpi{k}{\subName}} \hpi{k}{\into{t[u_i/x_i]}} \\
\sub{\seq{t_1, \dots, t_n}}{\ind{u}} := \hcomp{\pair{\into{t_1}, \dots, \into{t_n}}}{\into{u_i}} \XRA{\postName } \pair{\hcomp{\into{\ind{t}}}{\into{u_i}}} \XRA{\pair{\subName, \dots, \subName}} \pair{\into{\ind{t}[u_i/x_i]}}
\end{gather*}
\end{small}
and 
\begin{small}
\begin{align*}
\cont{\app{t}{u}}{\ind{v}} := \hcomp{\heval{\into{t}, \into{u}}}{\into{\ind{v}}} &\XRA{\assoc{}} \heval{\hcomp{\into{t}}{\into{\ind{v}}}, \hcomp{\into{u}}{\into{\ind{v}}}} \\ 
		&\XRA{\heval{\contName, \contName}} \heval{\into{t[v_j/y_j]}}, {\into{u[v_j/y_j]}}  \\[8pt]
\sub{\lam{x}{t}}{\ind{u}} := \hcomp{\lam{x}{\into{t}}}{\into{\ind{v}}} &\XRA{\pushName} \lam{x}{\hcomp{\into{t}}{x, \wkn{\into{u}}{x}}} \\ 
		&\XRA{\lam{x}{\hcomp{\into{t}}{x, \cont{u}{\mathrm{inc}_x}}}} \lam{x}{\hcomp{\into{t}}{x, \into{u}}} \\ 					&\XRA{\lam{x}{\subName}} \lam{x}{\into{t[x / x, u_i/x_i]}}
\end{align*}
\end{small}
\end{myconstr}

With $\subName$ in hand we can extend the mapping $\into{-}$ to all rewrites. 

\begin{myconstr}
Extend Construction~\ref{constr:ccc:into-terms} to a map on rewrites by extending the definition for $\hir(\graph)$:
\begin{small}
\begin{align*}
\into{\etaTimes{t}} &:= \etaTimes{\into{t}} \\
\into{\epsilonTimesInd{k}{t_1, \dots, t_n}} &:= \epsilonTimesInd{k}{\into{t_1}, \dots, \into{t_n}} \\
\into{\pi_k(\tau)} &:= \hcomp{\pi_k}{\into{\tau}} \\
\into{\seq{\sigma_1, \dots, \sigma_n}} &:= \pair{\into{\sigma_1}, \dots, \into{\sigma_n}} \\
\into{\etaExp{t}} &:= \into{t} \XRA{\etaExp{\into{t}}} \lam{x}{\heval{\wkn{\into{t}}{x}, x}} \XRA{\lam{x}{\heval{\contName, x}}} \lam{x}{\heval{\into{t},x}} \\
\into{\genEpsilonExp{x \bind t, u}} &:= \heval{\lam{x}{\into{t}}, \into{u}} \XRA{\genEpsilonExp{x \bind \into{t}, \into{u}}} \hcomp{\into{t}}{x_1 \mapsto x_1, \dots, x_n \mapsto x_n, x \mapsto \into{u}} \XRA{\subName} \into{t[u/x]} \\
\into{\app{\tau}{\sigma}} &:= \heval{\into{t}, \into{u}} \XRA{\heval{\into{\tau}, \into{\sigma}}} \heval{\into{t'}, \into{u'}} \\
\into{\lam{x}{\tau}} &:= \lam{x}{\into{t}} \XRA{\lam{x}{\into{\tau}}} \lam{x}{\into{t'}} 
\end{align*}
\end{small}
\qedhere
\end{myconstr}

This definition on rewrites continues to respect typings and the equational theory. 

\begin{prooflesslemma} \todo{check this carefully!}
For any 2-multigraph $\graph$,
\begin{enumerate}
\item For all derivable rewrites $\tau, \tau'$ in $\hirCCC(\graph)$, if $\tau \aeq \tau'$ then $\into{\tau} \aeq \into{\tau}$, 
\item If $\Gamma \vdash \tau : \rewrite{t}{t'} : B$ in $\hirCCC(\graph)$ then $\Gamma \vdash \into{\tau} : \rewrite{\into{t}}{\into{t'}} : B$ in $\langCartClosed(\graph)$,
\item If $\Gamma \vdash \tau \equiv \tau' : \rewrite{t}{t'} : B$ in $\hirCCC(\graph)$ then $\Gamma \vdash \into{\tau} \equiv \into{\tau'} : \rewrite{\into{t}}{\into{t'}} : B$ in $\langCartClosed(\graph)$. \qedhere
\end{enumerate}
\end{prooflesslemma}

As one would expect, $\subName$ and $\contName$ coincide where the terms being substituted are all variables. 

\begin{mylemma} \label{lem:out-cont-coincide}
If $\Gamma \vdash \into{t} : B$ and $r : \Gamma \to \Delta$ is a context renaming, then 
\[
\Delta \vdash \sub{t}{r(\ind{x})} \equiv \cont{t}{r} : \hcomp{\into{t}}{x_i \mapsto r(x_i)} \To \into{t} : B
\]
\begin{proof}
By induction on the derivation of $t$: comparing the cases one-by-one, the equality is immediate.
\end{proof}
\end{mylemma}

Moreover, all the work witnessed by $\subName$ is strictified under the $\out{({-})}$ maps. 

\begin{mylemma} \label{lem:out-sub-is-id}
If $\context \vdash t : B$ and $\subContext$ are derivable judgements in $\langCartClosed(\graph)$, then the judgement
\[
\Delta \vdash \out{\sub{t}{\ind{u}}} \equiv \id_{\out{t}[\out{u_i}/x_i]} : \rewrite{\out{t}[\out{u_i}/x_i]}{\out{t}[\out{u_i}/x_i]} : B
\]
is derivable in $\hirCCC(\graph)$.
\begin{proof}
By induction on the derivation of $t$; for the \rulename{pair} and \rulename{lam} cases we use Lemma~\ref{lem:out-push-post-id}.
\end{proof}
\end{mylemma}

As in the biclone case, proving that $\into{-}$ forms a pseudofunctor is more subtle than for $\out{({-})}$. Once again it is clear that $\into{-}$ strictly preserves the identity, so the difficulty is showing that $\subName$ satisfies the required properties to make $(\into{-}, \subName, \id)$ a pseudofunctor. As a first step, we establish some auxiliary properties that will be of use in the main proof. 

It is convenient to prove the axioms first; these make the naturality laws easier to check. We begin by observing that one of the axioms holds by definition: if $x_1 : A_1, \dots, x_n : A_n \vdash x_k : A_k$ and $(\Delta \vdash \into{u_i} : A_i)_{i=1,\dots,n}$ it follows immediately that $\sub{x_k}{\ind{u}} \equiv \indproj{k}{\ind{u}}$ for $k=1,\dots,n$. The next lemma establishes the other unit law.

\begin{mylemma} \label{lem:sub-pseudofun-unit}
If $\context \vdash \into{t} : B$ 
\[
\context \vdash \sub{t}{x_1, \dots, x_n} \vert \subid{\into{t}} \equiv \id_{\into{t}} : \rewrite{\into{t}}{\into{t}} : B
\]
\begin{proof}
By induction on the structure of $t$. The cases are all immediate from the inductive hypothesis and the definition except for the lambda abstraction case, where one must use the fact that $\sub{x_k}{x_1, \dots, x_n} := \indproj{k}{\ind{x}}$.
\end{proof}
\end{mylemma}

The associativity law is more difficult. We begin with a lemma that we will use in the lambda abstraction case.

%
% set all the arrows in tikz-cd diagrams in this block to be Rightarrow
{\tikzcdset{arrow style=tikz, arrows={Rightarrow}}
\begin{mylemma} \label{lem:lemma-for-sub-assoc-law}
Suppose that $x_1 : A_1, \dots, x_n : A_n \vdash \into{t} : B$.
\begin{enumerate}
\item \label{c:variables-assoc-and-sub} The following diagram commutes:
\begin{td}
\wkn{\wkn{\into{t}}{x}}{x} \arrow[Rightarrow]{r}{\assoc{}} \arrow[swap, Rightarrow]{d}{\wkn{\subName}{x}} &
\hcomp{\into{t}}{\hcomp{\ind{x}}{\ind{x}}} \arrow[Rightarrow]{r}{\hcomp{\into{t}}{\indproj{i}{}}} &
\hcomp{\into{t}}{\ind{x}} \arrow[Rightarrow]{d}{\subName} \\
\wkn{\into{t}}{x} \arrow[swap, Rightarrow]{rr}{\subName} &
\: &
\into{t}
\end{td}
\item \label{c:weakening-assoc-and-sub} If $(\Delta, x : A \vdash \into{u_i} : A_i)_{i=1,\dots,n}$, then
\begin{small}
\begin{td}
\hcomp{\wkn{t}{x}}{x_i \mapsto \into{u_i}, x \mapsto x} \arrow{r}{\assoc{}} \arrow[swap, Rightarrow]{d}{\hcomp{\subName}{x_i \mapsto \into{u_i}, x \mapsto x}} &
\hcomp{\into{t}}{\hcomp{\ind{x}}{x_i \mapsto \into{u_i}, x \mapsto x}} \arrow[Rightarrow]{r}{\hcomp{\into{t}}{\indproj{i}{}}} &
\hcomp{\into{t}}{x_i \mapsto \into{u_i}} \arrow[Rightarrow]{d}{\subName} \\
\hcomp{\into{t}}{x_i \mapsto \into{u_i}, x \mapsto x} \arrow[swap, Rightarrow]{rr}{\subName} &
\: &
\into{t[u_i/x_i]}
\end{td}
\end{small}
\end{enumerate}
\begin{proof}
By induction on the derivation of $\into{t}$. For both~(\ref{c:variables-assoc-and-sub}) and~(\ref{c:weakening-assoc-and-sub}) the difficult case is lambda abstraction. In each case, one unfolds the definition of $\subName$ and applies naturality so that one can use Lemma~\ref{lem:properties-of-push}(\ref{c:push-and-assoc}) and the inductive hypothesis. For~(\ref{c:variables-assoc-and-sub}) the rest of the proof is a standard diagram chase using naturality and coherence; for~(\ref{c:weakening-assoc-and-sub}) one also needs to use the result from~(\ref{c:variables-assoc-and-sub}).
\end{proof}
\end{mylemma}

We now turn to proving the associativity law.

\begin{mylemma} \label{lem:sub-pseudofun-assoc}
If $\context \vdash \into{t} : C$, $(y_1 : B_1, \dots, y_m : B_m \vdash \into{u_i} : A_i)_{i=1,\dots,n}$ and $(\Sigma \vdash \into{v_j} : B_j)_{j=1, \dots, m}$ in $\langCartClosed(\graph)$, then 
\begin{td}[column sep = huge]
 \hcompthree{\into{t}}{\into{u_i}}{\into{v_j}} \arrow[Rightarrow]{r}{\hcomp{\sub{t}{\ind{u}}}{v_j}}  \arrow[swap]{d}{\assoc{}} &
 \hcomp{\into{t[u_i / x_i]}}{\into{v_j}} \arrow[Rightarrow]{dd}{\sub{t[u_i/x_i]}{\ind{v}}}  \\
 \hcomp{\into{t}}{\hcomp{\into{u_i}}{\into{v_j}}} \arrow[swap, Rightarrow]{d}{\hcomp{\into{t}}{\sub{u_i}{\ind{v}}}} &
 \: \\
 \hcomp{\into{t}}{\into{u_i[v_j / y_j]}} \arrow[swap, Rightarrow]{r}{\sub{t}{\ind{u}[v_j/y_j]}} &
 \into{t\big[u_i[v_j/y_j]/x_i\big]}
\end{td}
\begin{proof}
We induct on the derivation of $t$. The \rulename{var}, \rulename{const}, \rulename{proj} and \rulename{app} cases are straightforward, while for \rulename{pair} one also makes use of the compatibility law between $\assoc{}$ and $\postName$ \big(Lemma~\ref{lem:properties-of-post}(\ref{c:post-and-assoc})\big). As usual, the difficult case is \rulename{lam}. The strategy is the same to that for Lemma~\ref{lem:lemma-for-sub-assoc-law}: one employs Lemma~\ref{lem:properties-of-push}(\ref{c:push-and-assoc}) and naturality so that one can apply the inductive hypothesis. To deal with the $\lam{x}{\hcomp{\into{t}}{\contName, x}}$ component of the definition of $\sub{\lam{x}{t}}{\ind{u}}$, one uses the preceding lemma.
\end{proof}
\end{mylemma}

A useful corollary of the associativity law is the following.

\begin{prooflesscor} \label{cor:sub-assoc-phi}
If $x_1 : A_1, \dots, x_n : A_n \vdash \into{t} : B$ and $(\Delta \vdash \into{u_i} : A_i)_{i=1,\dots, n}$, then
\begin{td}
\hcomp{\wkn{\into{t}}{x}}{x_i \mapsto \wkn{\into{u_i}}{x}, x \mapsto x} \arrow{r}{\hcomp{\subName}{\subName, x}} \arrow[swap]{d}{\phiCell{2}{}} &
\hcomp{\into{t}}{x_i \mapsto \into{u_i}, x \mapsto x} \arrow{dd}{\subName} \\
\wkn{\hcomp{\into{t}}{x_i \mapsto \into{u_i}}}{x} \arrow[swap]{d}{\wkn{\subName}{x}} &
\: \\
\wkn{\into{t[u_i/x_i]}}{x} \arrow[swap]{r}{\subName} &
\into{t[u_i/x_i]}
\end{td}
\end{prooflesscor}
}

We now prove the naturality of $\subName$.

%
% set all the arrows in tikz-cd diagrams in this block to be Rightarrow
{\tikzcdset{arrow style=tikz, arrows={Rightarrow}}
\begin{mylemma} \label{lem:sub-nat}
Suppose that $x_1 : A_1, \dots, x_n : A_n \vdash \tau : \rewrite{t}{t'} : B$ and $(\Delta \vdash \sigma_i : \rewrite{u_i}{u_i'} :A_i)_{i=1,\dots,n}$. Then the following diagrams commute
\begin{center}
\begin{minipage}{0.45\textwidth}
\begin{equation} \label{diag:sub-nat-tau}
\begin{small}
\begin{tikzcd}
\hcomp{\into{t}}{\into{\ind{u}}} \arrow{r}{\subName} \arrow[swap]{d}{\hcomp{\into{\tau}}{\into{\ind{u}}}} &
\into{t[u_i/x_i]} \arrow{d}{\into{\tau[u_i/x_i]}} \\
\hcomp{\into{t'}}{\into{\ind{u}}} \arrow[swap]{r}{\subName} &
\into{t'[u_i/x_i]}
\end{tikzcd}
\end{small}
\end{equation}
\end{minipage}
\:\:
\begin{minipage}{0.45\textwidth}
\begin{equation} \label{diag:sub-nat-sigma}
\begin{small}
\begin{tikzcd}
\hcomp{\into{t}}{\into{\ind{u}}} \arrow{r}{\subName} \arrow[swap]{d}{\hcomp{\into{t}}{\into{\ind{\sigma}}}} &
\into{t[u_i/x_i]} \arrow{d}{\into{t[\sigma_i/x_i]}} \\
\hcomp{\into{t}}{\into{\ind{u}'}} \arrow[swap]{r}{\subName} &
\into{t[u_i'/x_i]}
\end{tikzcd}
\end{small}
\end{equation}
\end{minipage}
\end{center}
and hence so does the diagram
\begin{td}
\hcomp{\into{t}}{\into{\ind{u}}} \arrow{r}{\subName} \arrow[swap]{d}{\hcomp{\into{\tau}}{\into{\ind{\sigma}}}} &
\into{t[u_i/x_i]} \arrow{d}{\into{\tau[\sigma_i/x_i]}} \\
\hcomp{\into{t'}}{\into{\ind{u}'}} \arrow[swap]{r}{\subName} &
\into{t'[u_i'/x_i]}
\end{td}
\begin{proof}
For~(\ref{diag:sub-nat-sigma}) we induct on the structure of $t$: the result follows from the naturality of the structural maps (for \rulename{var}, \rulename{const}, \rulename{proj} and \rulename{app}), the naturality of $\postName$ and $\pushName$ (for \rulename{pair} and \rulename{lam}, respectively), and the inductive hypothesis.

For~(\ref{diag:sub-nat-tau}) we induct on the derivation of $\tau$. As usual the difficult cases are those for exponential structure. For $\etaExp{}$ one uses the compatibility of $\etaExp{}$ and $\pushName$ \big(Lemma~\ref{lem:properties-of-push}(\ref{c:push-with-etaexp})\big) and naturality, and then Corollary~\ref{cor:sub-assoc-phi} to deal with the $\lam{x}{\heval{\contName, x}}$ component. For $\genEpsilonExp{}$ one uses the associativity law (Lemma~\ref{lem:sub-pseudofun-assoc}) and the compatibility of $\pushName$ and $\assoc{}$ \big(Lemma~\ref{lem:properties-of-push}(\ref{c:push-and-assoc})\big).
\end{proof}
\end{mylemma}

Putting all this together, we see that $\into{-}$ does indeed extend to a pseudofunctor.

\begin{mypropn}
The mapping $\into{-}$ extends to a pseudofunctor $\hirCCCSyn(\graph) \to \termCatCCC(\graph)$.
\begin{proof}
By Lemmas~\ref{lem:sub-pseudofun-unit},~\ref{lem:sub-pseudofun-assoc} and~\ref{lem:sub-nat}.
\end{proof}
\end{mypropn}
}

\subsubsection{Defining the pseudonatural transformations}

The next part of the construction is to define a pair of invertible pseudonatural transformations \mbox{$\into{-} \circ \out{({-})} \iso \id_{\termCatCCC(\graph)}$} and $\out{({-})} \circ \into{-} \iso \id_{\hirCCCSyn(\graph)}$. For the latter we can in fact take the identity.

\begin{mylemma} \label{lem:out-into-is-id}
The composite pseudofunctor $\out{({-})} \circ \into{-}$ is exactly the identity on $\hirCCCSyn(\graph)$. 
\begin{proof}
On objects this is trivial; on terms we have the following:
\begin{gather*}
x_k \mapsto x_k \mapsto x_k \\
c(u_1, \dots, u_n) \mapsto \hcomp{c}{\into{u_1}, \dots, \into{u_n}} \mapsto c(x_1, \dots, x_n)[\out{\into{u_i}}/x_i] \\[8pt]
\pi_k(t) \mapsto \hpi{k}{\into{t}} \mapsto \pi_k(p)[\out{\into{t}} / p] \\
\seq{t_1, \dots, t_n} \mapsto \pair{\into{t_1}, \dots, \into{t_n}} \mapsto \seq{\out{\into{t_1}}, \dots, \out{\into{t_n}}} \\[8pt]
\app{t}{u} \mapsto \heval{\into{t}, \into{u}} \mapsto (\app{f}{a})[\out{\into{t}} / f, \out{\into{u}} / a] \\
\lam{x}{t} \mapsto \lam{x}{\into{t}} \mapsto \lam{x}{\out{\into{t}}}
\end{gather*}
so the claim holds by induction. For rewrites the cases are all similar except for the unit and counit of exponentials; for these one uses Lemmas~\ref{lem:out-sub-is-id} and~\ref{lem:out-cont-coincide}.
\end{proof}
\end{mylemma}

We therefore turn to the composite $\into{-} \circ \out{({-})}$. Following our approach for biclones, we define an invertible pseudonatural transformation $\reduceName$. For 1-cell components we take the identity. For 2-cells we need to give a rewrite filling
%
% set all the arrows in tikz-cd diagrams in this block to be Rightarrow
{\tikzcdset{arrow style=tikz, arrows={Rightarrow}}
\begin{td}[column sep = huge]
\Gamma \arrow{r}[yshift=2mm]{(\Gamma \vdash t_j : B_j)_{j=1,\dots,m}} \arrow[swap]{d}{\Id_\Gamma} \arrow[phantom]{dr}[description]{\twocellIso{\reduceName}} &
\Delta \arrow{d}{\Id_\Delta} \\
\Gamma \arrow[swap]{r}[yshift=-2mm]{(\Gamma \vdash \into{\out{t_j}} : B_j)_{j=1,\dots,m}} &
\Delta
\end{td}
for each morphism $(\Gamma \vdash t_j : B_j)_{j=1,\dots,m} : \Gamma \to \Delta$, where $\Delta := (y_j :B_j)_{j=1,\dots,m}$. It suffices to work pointwise and we may use the coherence theorem for biclones to treat $\Id_\Gamma$ and $\Id_\Delta$ as strict identities. Thus, the problem reduces to defining a family of rewrites filling
\begin{td}[column sep = huge]
\Gamma \arrow{r}{\Gamma \vdash t : B} \arrow[swap, equals]{d}{} \arrow[phantom]{dr}[description]{\twocellIso{\reduceName}} &
B \arrow[equals]{d}{} \\
\Gamma \arrow[swap]{r}{\Gamma \vdash \into{\out{t}} : B} &
B
\end{td}
}
For this we extend the construction for biclones.

\begin{myconstr}
Define an invertible rewrite $\reduceName$ with signature
\begin{center}
\unaryRule	{\Gamma \vdash t : B}
{\Gamma \vdash \reduce{t} : \rewrite{t}{\into{\out{t}}} :  B}
{}
\end{center}
by extending Construction~\ref{constr:biclone-reduce} with the following rules:
\begin{gather*}
\reduce{\pi_k(p)} := \pi_k(p) \XRA{\subid{}} \hpi{k}{p} \\
\reduce{\pair{t_1, \dots, t_n}} := \pair{t_1, \dots, t_n} \XRA{\pair{\reduceName, \dots, \reduceName}} \pair{\into{\out{t_1}}, \dots, \into{\out{t_n}}} \\
\reduce{\evalterm(f,a)} := \evalterm(f,a) \XRA{\subid{}} \heval{f,a} \\
\reduce{\lam{x}{t}} := \lam{x}{t} \XRA{\lam{x}{\reduce{t}}} \lam{x}{\into{\out{t}}}
\end{gather*}
\end{myconstr}

Our first observation is that $\reduceName$ does indeed provide a notion of \emph{normalisation}.

\begin{mylemma}
For any $\Gamma \vdash t : B$ derivable in $\hirCCC(\graph)$, the judgement
\[
\Gamma \vdash \reduce{\into{t}} \equiv \id_{\into{t}} : \rewrite{\into{t}}{\into{t}} : B
\]
is derivable in $\langCartClosed(\graph)$. 
\begin{proof}
An easy induction on the structure of $t$.
\end{proof}
\end{mylemma}

The identity and associativity laws required for $\reduceName$ to be a pseudonatural transformation hold immediately from the definition, so it remains to show that $\reduceName$ is a natural family of 2-cells. For this we begin with the following lemma establishing some results that will be of use for the proof.

\begin{mylemma} \quad \label{lem:results-for-reduce-nat}
\begin{enumerate}
\item \label{c:sub-with-beta-and-epsilon} For any context $\Gamma := (x_i : A_i)_{i=1,\dots,n}$ and derivable judgement $\Gamma, x : A \vdash \into{u} : B$, 
\begin{td}[column sep = huge]
\heval{\wkn{(\lam{x}{\into{u})}}{x}, x} \arrow{r}{\heval{\subName, x}} \arrow[Rightarrow, swap]{d}{\epsilonExpRewr{\into{u}}} &
\heval{\lam{x}{\into{u}}, x} \arrow[Rightarrow]{d}{\genEpsilonExp{}} \\
\into{u} &
\hcomp{\into{u}}{\id_\Gamma, x \mapsto x} \arrow[Rightarrow]{l}{\subName}
\end{td}
\item \label{c:reduce-with-subid} For any derivable judgement $\context \vdash t : B$ in $\langCartClosed$, 
\begin{td}
t \arrow[Rightarrow]{r}{\subid{}} \arrow[swap, Rightarrow]{dr}{\reduceName} &
\hcomp{t}{x_i \mapsto x_i} \arrow[Rightarrow]{d}{\reduceName} \\
\: &
\into{\out{t}}
\end{td}
\end{enumerate}
\begin{proof}
We prove~(\ref{c:sub-with-beta-and-epsilon}) directly by unfolding the composite term and using the the compatibility between $\pushName$ and $\subid{}$ \big(Lemma~\ref{lem:properties-of-push}(\ref{c:push-and-subid})\big).  For~(\ref{c:reduce-with-subid}) the only difficult case is lambda abstraction, where one also needs to make use of the compatibility of $\pushName$ and $\subid{}$ as well as the inductive hypothesis.
\end{proof}
\end{mylemma}

Now we turn to proving naturality.

\begin{mylemma}
The following rule is admissible in $\langCartClosed(\graph)$:
\begin{center}
\unaryRule	{\Gamma \vdash \tau : \rewrite{t}{t'} : B}
{\Gamma \vdash \into{\out{\tau}} \vert \reduce{t} \equiv \reduce{t'} \vert \tau : \rewrite{t}{\into{\out{t'}}} :  B}
{}
\end{center}
\begin{proof}
We induct on the derivation of $\tau$. For the structural isomorphisms, the $\indproj{k}{}$ case holds immediately from naturality. For $\subid{}$ we apply Lemma~\ref{lem:results-for-reduce-nat}(\ref{c:sub-with-beta-and-epsilon}), while for $\assoc{}$ we use both naturality and the associativity law for $\subName$ (Lemma~\ref{lem:sub-pseudofun-assoc}). The identity and two composition operations are straightforward. 

For product structure, the $\epsilonTimesInd{k}{}$ holds by naturality of $\epsilonTimesInd{k}{}$; for $\transTimes{\alpha_1, \dots, \alpha_n}$ we calculate that 
\begin{align*}
\epsilonTimesInd{k}{\into{\out{\ind{t}}}} &\vert \hpi{k}{\into{\out{\transTimes{\alpha_1, \dots, \alpha_n}}} \vert \reduce{u}}  \\
	&\equiv \epsilonTimesInd{k}{\into{\out{\ind{t}}}} \vert \hpi{k}{\pair{\into{\out{\alpha_1}}, \dots, \into{\out{\alpha_n}}} \vert \etaTimes{\into{\out{u}}}} \vert \hpi{k}{\reduce{u}} \\
	&\equiv \into{\out{\alpha_k}} \vert \epsilonTimesInd{k}{\hcomp{\ind{\pi}}{\into{\out{u}}}} \vert \hpi{k}{\etaTimes{\into{\out{u}}}} \vert \hpi{k}{\reduce{u}} \\
	&\equiv \into{\out{\alpha_k}} \vert \hpi{k}{\reduce{u}}  \qquad \text{by the triangle law} \\
	&\overset{\text{IH}}{\equiv} \reduce{t_k} \vert \alpha_k  \\
	&\equiv  \reduce{t_k} \vert \epsilonTimesInd{k}{\ind{t}} \vert \hpi{k}{\transTimes{\alpha_1, \dots, \alpha_n}}  \\
	&\equiv \epsilonTimesInd{k}{\into{\out{\ind{t}'}}} \vert \hpi{k}{\pair{\reduce{t_1}, \dots, \reduce{t_n}} \vert \transTimes{\alpha_1, \dots, \alpha_n}} 
\end{align*}
Applying the universal property of $\transTimes{\alpha_1, \dots, \alpha_n}$, we obtain the required equality. 

For exponential structure, one uses Lemma~\ref{lem:results-for-reduce-nat}(\ref{c:sub-with-beta-and-epsilon}) for the $\epsilonExpRewr{}$ case and Lemma~\ref{lem:results-for-reduce-nat}(\ref{c:reduce-with-subid}) for the $\transExp{x \bind \alpha}$ case. 
\end{proof}
\end{mylemma}

\begin{prooflesscor}
$(\Id, \reduceName)$ forms an invertible pseudonatural transformation $\id_{\termCatCCC(\graph)} \XRA{\iso} \into{-} \circ \out{({-})}$. 
\end{prooflesscor}

Hence, together with Lemma~\ref{lem:out-into-is-id}, we obtain a biequivalence.

\begin{prooflesscor}
The pseudofunctors $\into{-} : \hirCCCSyn(\graph) \leftrightarrows \termCatCCC(\graph) : \out{({-})}$ and the pseudonatural transformation $(\Id, \reduceName)$ form a biequivalence $\hirCCCSyn(\graph) \simeq \termCatCCC(\graph)$. By Lemma~\ref{lem:bicat-to-cartclosedbicat-equivalence-lift}, this lifts canonically to a CC-biequivalence.
\end{prooflesscor}


==> extension-pseudofunctor.tex <==
\begin{figure*}[!h]
\begin{minipage}{\textwidth}
{\small
\begin{mdframed}
\begin{align*} 
h\sem{B} &:= h(B) \qquad \text{on base types} \\
h\sem{\prodop_n(B_1, \dots, B_n)} &:= \prodop_{i=1}^n h\sem{B_i} \\
h\sem{\exptype{A}{B}} &:= \expobj{h\sem{A}}{h\sem{B}}  \\
h\sem{x_1 : A_1, \dots, x_n : A_n} &:= \prodop_{i=1}^n h\sem{A_i} \qquad \text{on $n$-ary contexts} \\[5pt]
h\sem{x_1 : A_1, \dots, x_n : A_n \vdash x_k :A_i} &:= \pi_k^{A_1, \dots, A_n} \\ 
h\sem{x_1 : A_1, \dots, x_n : A_n \vdash c(x_1, \dots, x_n) : B} &:= h(c) \qquad \text{ for } c \in \graph(\ind{A};B) \\ 
h\sem{\Delta \vdash \hcomp{t}{x_i^{A_i} \mapsto u_i}_{i=1}^n : B} &:= h\sem{x_1 : A_1, \dots, x_n : A_n \vdash t : B} \circ \seq{h\sem{\Delta \vdash u_i : A_i}}_{i = 1, \dots, n} \\ 
h\sem{\Gamma \vdash \pair{t_1, \dots, t_n} : \prodop_n(B_1, \dots, B_n)} &:= \seq{h\sem{\Gamma \vdash t_1 : B_1,},\dots, h\sem{\Gamma \vdash t_n : B_n}} \\
h\sem{p : \prodop_n(B_1, \dots, B_n) \vdash \pi_k(p) : B_k} &:= \pi_k^{B_1, \dots, B_n} \\
h\sem{f : \exptype{A}{B}, a : A \vdash \evalterm(f,a) : B} &:= \eval_{A,B} \\
h\sem{\Gamma \vdash \lam{x}{t} : \exptype{A}{B}} &:= \lambda\big(h\sem{\Gamma, x : A \vdash t : B}\big) \\[5pt]
h\sem{\Gamma \vdash \id_t : \rewrite{t}{t} : B} &:= \id_{h\sem{\Gamma \vdash t : B}} \\
h\sem{x_1 : A_1, \dots, x_n : A_n \vdash \sigma(\ind{x}) : \rewrite{c(\ind{x})}{c'(\ind{x})} : B} &:= h(\sigma) \qquad \text{ for } \sigma \in \graph(\ind{A}, B)(c,c')  \\
h\sem{\Gamma \vdash \epsilonTimesInd{k}{t_1, \dots, t_n} : \rewrite{\hcomp{\pi_k}{\pair{t_1, \dots, t_n}}}{t_k} : B_k} &:= \epsilonTimesInd{k}{h\sem{t_1}, \dots, h\sem{t_n}} \\
h\sem{\Gamma \vdash \transTimes{\alpha_1, \dots, \alpha_n} : \rewrite{u}{\pair{t_1, \dots, t_n}} : \prodop_n(B_1, \dots, B_n)} &:= \transTimes{h\sem{\Gamma \vdash \alpha_i : \rewrite{\hcomp{\pi_i}{u}}{t_i} : B_i}}_{i=1, \dots, n} \\
h\sem{\Gamma, x : A \vdash \epsilonExpRewr{t} : \rewrite{\genevalterm{\wkn{(\lam{x}{t})}{x}, x}}{t} : B} &:= \epsilon_{h\sem{\Gamma, x : A \vdash t : B}} \\
h\sem{\Gamma \vdash \transExp{x \bind \alpha} : \rewrite{u}{\lam{x}{t}} : \exptype{A}{B}} &:= \transExp{h\sem{\Gamma, x : A \vdash \alpha : \rewrite{\genevalterm{\wkn{u}{x}, x}}{t} : B}} \\
h\sem{\Gamma \vdash \tau' \vert \tau : \rewrite{t}{t''} : B} &:= h\sem{\Gamma \vdash \tau' : \rewrite{t'}{t''} : B} \vert h\sem{\Gamma \vdash \tau : \rewrite{t}{t'} : B} \\
h\sem{\Delta \vdash \hcomp{\tau}{x_i^{A_i} \mapsto \sigma_i}_{i= 1}^n : \rewrite{\hcomp{t}{x_i^{A_i} \mapsto u_i}_{i= 1}^n}{\hcomp{t'}{x_i^{A_i} \mapsto u_i'}_{i= 1}^n} : B} &:= h\sem{x_1 : A_1, \dots, x_n : A_n \vdash \tau : \rewrite{t}{t'} : B} \circ \: \\ 
		&\hspace{35mm} \circ \seq{h\sem{\Delta \vdash \sigma_i : \rewrite{u_i}{u_i'} : A_i}}_{i=1, \dots, n}
\end{align*} 
\caption{The extension CC-pseudofunctor \label{fig:extension-pseudofunctor}}
\end{mdframed}
}
\end{minipage}
\end{figure*}

==> prod-eq-th.tex <==
\begin{rules}

\input{rules/cart/trans-ump}

\caption{Universal property of $\transTimes{-}$}
\end{rules}

\subsubsection{Congruence and invertibility rules}

\begin{rules}
	\input{rules/cart/invertibility-congruences}

	\caption{Invertibility rules for pseudo-product structure}
\end{rules}

==> rules-bicat.tex <==
%\documentclass{report}
%
%\input{macros}
%\usepackage{graphicx}
%\usepackage{a4wide}
%\usepackage[footskip=1.5in]{geometry}
%
%\begin{document}

\setcounter{figure}{0} 
\renewcommand\thefigure{\thesection.\arabic{figure}}      

\subsection{The rules of $\langBicat(\graph)$}  \label{sec:rules}

Fix some 2-graph $\graph$ with nodes $\nodes{\graph}$ and hom-graphs $\graph(X, Y)$. 

%\subsection{Contexts}

\begin{figure*}
{\small	
	
\begin{rules}
\input{rules/bicat/contexts}
\end{rules}

%\subsection{Terms}

\begin{rules}

\input{rules/bicat/terms}

\caption{Rules for terms}
\end{rules}

%\pagebreak
%\subsection{Rewrites}

\begin{rules}
\input{rules/bicat/structural-rewrites}

\input{rules/bicat/constant-and-id-rewrites}

\input{rules/bicat/constructors-on-rewrites}

\caption{Introduction rules and constructors on rewrites}
\end{rules}

}
\end{figure*}

%\clearpage
%\pagebreak
%\subsection{The equational theory}

%\subsubsection{Functorality of the constructors}

\begin{figure*}
	
{\small	
\begin{rules}
\input{rules/bicat/categorical-vert-comp}
\caption{Categorical structure of vertical composition}
\end{rules}

\begin{rules}
		
\input{rules/bicat/hcomp-vcomp-preservation}

\caption{Preservation rules}
\end{rules}

%\subsubsection{Biclone laws}

\begin{rules}
\input{rules/bicat/biclone-nat}

\caption{Naturality rules on structural rewrites}
\end{rules}


\begin{rules}
\input{rules/bicat/biclone-laws}

\caption{Compatibility laws}
\end{rules}
%\end{figure*}

%\pagebreak
%\subsubsection{Invertibility}

%\begin{figure*}
\begin{rules}
\input{rules/bicat/invertibility}

\caption{Invertibility of basic rewrites}
\end{rules}

%\pagebreak
%\subsubsection{Congruence rules}

\begin{rules}
\input{rules/bicat/congruence}
\caption{Congruence rules}
\end{rules}
}
\end{figure*}

%\end{document}


==> rules-cart.tex <==
%\documentclass{report}
%
%% packages
%\usepackage{etex}
%\usepackage{amsmath}
%\usepackage{amssymb}
%\usepackage{amsthm}
%\usepackage{amsfonts}
%\usepackage{mathtools}
%\usepackage{mathabx}
%\usepackage{bbold}
%\usepackage{parskip}
%\usepackage{amscd}
%\usepackage{thmtools}
%\usepackage{rotating} % for turning the \corner symbol
%\usepackage{tikz-cd} % for commutative diagrams
%\usepackage{bussproofs} % for proof trees
%\usepackage{stmaryrd} % for semantics brackets
%\usepackage{microtype}
%\usepackage{enumitem}
%\usepackage{graphicx}
%\usepackage{mdframed} % for putting boxes round things
%\usepackage{multicol} 
%\usepackage{accents} % for thicker widebar
%\usepackage[refpage]{nomencl} % for the index of notation
%% \usepackage{showlabels} % for putting label names in the marginpar
%%\renewcommand{\showlabelfont}{\scriptsize}
%\usepackage{tabulary}
%
%\input{macros}
%\usepackage{graphicx}
%\usepackage{a4wide}
%\usepackage[footskip=1.5in]{geometry}
%
%\begin{document}

\setcounter{figure}{0} 
\renewcommand\thefigure{\thesection.\arabic{figure}}      

\hide{\subsection{The rules of $\langCart(\graph)$}  \label{sec:rules-cart}

Fix a 2-multigraph $\graph$ with nodes $\nodes{\graph}$. Write $\widetilde{\nodes{\graph}}$ for the set generated by the grammar
\[
X_1, \dots, X_n ::= A \in \nodes{\graph} \st \textstyle{\prod_n}(X_1, \dots, X_n) \text{ for all } n \in \Nat 
\]
}
%\subsubsection{Contexts}

\begin{figure*}
	
{\small	
\begin{rules}
\input{rules/contexts}
			
\caption{Rules for contexts}
\end{rules}

%\subsubsection{Terms}

\begin{rules}
\input{rules/basic-terms}
\input{rules/cart/products-terms}

\caption{Rules for terms}
\end{rules}

%\pagebreak
%\subsubsection{Rewrites}

\begin{rules}

\input{rules/structural-rewrites}

\caption{Introduction rules on structural rewrites}
\end{rules}

\begin{rules}

\input{rules/basic-rewrites}

\input{rules/cart/products-rewrites}

\input{rules/rewrites-constructors}

\caption{Introduction rules on rewrites}
\end{rules}

\begin{rules}
	\input{rules/cart/invertibility-intro}	
	\caption{Introduction rules for pseudo-products structure}
\end{rules}
}
\end{figure*}

%\pagebreak
%\subsubsection{The equational theory}

%\subsubsection{Functorality of the constructors}

\clearpage
\begin{figure*}
{\small
\begin{rules}

\input{rules/categorical-vert-comp}
\caption{Categorical structure of vertical composition}
\end{rules}

\begin{rules}

\input{rules/interchange}

\caption{Preservation rules}
\end{rules}

%\pagebreak
%\subsubsection{Biclone laws}

\begin{rules}
\input{rules/structural-rewrites-nat}
\caption{Naturality rules on structural rewrites}
\end{rules}

\begin{rules}

\input{rules/biclone-laws}
\caption{Biclone laws}
\end{rules}
}
\end{figure*}

%\pagebreak
%\subsubsection{Rules for products}

\begin{figure*}
{\small
\begin{rules}

\input{rules/cart/trans-ump}

\caption{Universal property of $\transTimes{-}$}
\end{rules}

%\subsubsection{Congruence and invertibility rules}

\begin{rules}
	\input{rules/cart/invertibility-congruences}

	\caption{Invertibility rules for pseudo-product structure}
\end{rules}

\begin{rules}
	\input{rules/congruences}
	\input{rules/cart/extra-congruence}
	
	\caption{Congruence rules}
\end{rules}

\begin{rules}
	\input{rules/structural-rewrites-invertibility}
	
	\caption{Invertibility of structural rewrites}
\end{rules}

}
\end{figure*}
%\end{document}


==> rules-ccc.tex <==
%\documentclass{report}
%
%% packages
%\usepackage{etex}
%\usepackage{amsmath}
%\usepackage{amssymb}
%\usepackage{amsthm}
%\usepackage{amsfonts}
%\usepackage{mathtools}
%\usepackage{mathabx}
%\usepackage{bbold}
%\usepackage{parskip}
%\usepackage{amscd}
%\usepackage{thmtools}
%\usepackage{rotating} % for turning the \corner symbol
%\usepackage{tikz-cd} % for commutative diagrams
%\usepackage{bussproofs} % for proof trees
%\usepackage{stmaryrd} % for semantics brackets
%\usepackage{microtype}
%\usepackage{enumitem}
%\usepackage{graphicx}
%\usepackage{mdframed} % for putting boxes round things
%\usepackage{multicol} 
%\usepackage{accents} % for thicker widebar
%\usepackage[refpage]{nomencl} % for the index of notation
%% \usepackage{showlabels} % for putting label names in the marginpar
%%\renewcommand{\showlabelfont}{\scriptsize}
%\usepackage{tabulary}
%
%\input{macros}
%\usepackage{graphicx}
%\usepackage{a4wide}
%\usepackage[footskip=1.5in]{geometry}
%
%\begin{document}

\setcounter{figure}{0} 
\renewcommand\thefigure{\thesection.\arabic{figure}}      

\hide{\subsection{The rules of $\langCartClosed(\graph)$}  \label{sec:rules-cart-closed}

Fix a 2-multigraph $\graph$ with nodes $\nodes{\graph}$. Write $\widetilde{\nodes{\graph}}$ for the set generated by the grammar
\[
X_1, \dots, X_n, X, Y ::= A \in \nodes{\graph} \st \textstyle{\prod_n}(X_1, \dots, X_n) \text{ for all } n \in \Nat \st \exptype{X}{Y}
\]
The rules of $\langCartClosed(\graph)$ are all those of $\langCart(\graph)$ (with types given by $\widetilde{\nodes{\graph}}$), with the following additions.
}
%\subsection{Terms}

\begin{figure*}
{\small	
	
\begin{rules}
\input{rules/ccc/exponential-terms}
			
\caption{Introduction rules for terms}
\end{rules}

%\subsection{Rewrites}

\begin{rules}
\input{rules/ccc/exponential-rewrites}
		
\caption{Introduction rules on rewrites}
\end{rules}

\begin{rules}
\input{rules/ccc/invertibility-intro}
\caption{Introduction rules for pseudo-exponentials structure}
\end{rules}

%\subsection{The equational theory}

%\subsubsection{Rules for exponentials}

\begin{rules}
\input{rules/ccc/trans-ump}
\caption{Universal property of $\transExp{-}$}
\end{rules}

\begin{rules}
\input{rules/ccc/derived-intro}
\caption{Derived introduction rules}
\end{rules}

%\pagebreak
%\subsubsection{Congruence and invertibility rules}

\begin{rules}
	
\input{rules/ccc/invertibility-congruences}

\caption{Invertibility rules for pseudo-exponential structure}
\end{rules}

\begin{rules}
\input{rules/ccc/extra-congruence}

\caption{Congruence rules}
\end{rules}

}
\end{figure*}
%\end{document}


==> rules/bicat/biclone-laws.tex <==
\begin{prooftree} 
\AxiomC{$x : A \vdash t : B$} 
\AxiomC{$z : Z \vdash u : A$} 
\BinaryInfC{$z : Z \vdash \hcomp{t}{x \mapsto \proj{u}} \vert \assoc{t,x,u} \vert \hcomp{\subid{t}}{x \mapsto u} \equiv \id_{\hcomp{t}{x \mapsto u}} : \rewrite{\hcomp{t}{x \mapsto u}}{\hcomp{t}{x \mapsto u}} : B$} 
\end{prooftree} \vspace{\treeskip} 

\begin{footnotesize} 
\begin{prooftree} 
\AxiomC{$z : Z \vdash u : A$} 
\AxiomC{$x : A \vdash v : B$} 
\AxiomC{$y: B \vdash w : C$} 
\AxiomC{$c : C \vdash t : D$} 
\alwaysSingleLine 
\QuaternaryInfC{$z : Z \vdash \big(\hcomp{t}{c \mapsto \assoc{w, v, u}} \vert \assoc{t, \hcomp{w}{y \mapsto v}, u}\big) \vert \hcomp{\assoc{t, w, v}}{x \mapsto u} \equiv \assoc{t, w, \hcomp{v}{x \mapsto u}} \vert \assoc{\hcomp{t}{c \mapsto w}, v, u}$} 
\noLine 
\UnaryInfC{\hspace{0.40\textwidth}$: \rewrite{\hcomp{\hcomp{\hcomp{t}{c \mapsto w}}{y \mapsto v}}{x \mapsto u}}{\hcomp{t}{c \mapsto \hcomp{w}{y \mapsto \hcomp{v}{x \mapsto u}}}} : D$} 
\end{prooftree} 
\end{footnotesize} \vspace{\treeskip} 



==> rules/bicat/biclone-nat.tex <==
\unaryRule {x : A \vdash \tau : \rewrite{t}{t'} : B} 
{x : A \vdash \subid{t'} \vert \tau \equiv \hcomp{\tau}{x \mapsto x} \vert \subid{t} : \rewrite{t}{\hcomp{t'}{x \mapsto x}} : B} 
{$\subid{}$-nat} 

\unaryRule {z : Z \vdash \sigma : \rewrite{u}{u'} : A} 
{z : Z \vdash \proj{u} \vert \hcomp{x}{x \mapsto \sigma} \equiv \sigma \vert \proj{u} : \rewrite{\hcomp{x}{x \mapsto u}}{u'} : A} 
{$\proj{}$-nat} 

\begin{footnotesize} 
\begin{prooftree} 
\alwaysNoLine 
\AxiomC{$z : Z \vdash \mu : \rewrite{u}{u'} : A$} 
\AxiomC{$x : A \vdash \sigma : \rewrite{v}{v'} : B$} 
\AxiomC{$y : B \vdash \tau : \rewrite{t}{t'} : C$} 
\alwaysSingleLine 
\RightLabel{\scriptsize $\assoc{}$-nat} 
\TrinaryInfC{$z : Z \vdash \assoc{t', v', u'} \vert \hcomp{\hcomp{\tau}{y \mapsto \sigma}}{x \mapsto \mu} \equiv \hcomp{\tau}{y \mapsto \hcomp{\sigma}{x \mapsto \mu}} \vert \assoc{t, v, u}$} 
\noLine 
\UnaryInfC{\hspace{0.3\textwidth}$: \rewrite{\hcomp{\hcomp{t}{y \mapsto v}}{x \mapsto u}}{\hcomp{t'}{y \mapsto \hcomp{v'}{x \mapsto u'}}} : C$} 
\end{prooftree} 
\end{footnotesize}\vspace{\treeskip} 


==> rules/bicat/categorical-vert-comp.tex <==
\unaryRule	{z : Z \vdash \tau : \rewrite{t}{t'} : A}
			{z : Z \vdash \id_{t'} \vert \tau \equiv \tau  : \rewrite{t}{t'} : A}
			{$\id_t$-left-unit}

\unaryRule	{z : Z \vdash \tau : \rewrite{t}{t'} : A}
			{z : Z \vdash \tau \vert \id_t \equiv \tau : \rewrite{t}{t'} : A}
			{$\id_t$-right-unit}

\trinaryRule	{z : Z \vdash \tau'' : \rewrite{t''}{t'''} : A}
				{z : Z \vdash \tau' : \rewrite{t'}{t''} : A}
				{z : Z \vdash \tau : \rewrite{t}{t'} : A}
				{z : Z \vdash (\tau'' \vert \tau') \vert \tau \equiv \tau'' \vert (\tau' \vert \tau) : \rewrite{t}{t'''} : A}
				{$\vert$-assoc}

==> rules/bicat/congruence.tex <==
\unaryRule	{z : Z \vdash \tau : \rewrite{t}{t'} : A}
			{z : Z \vdash \tau \equiv \tau : \rewrite{t}{t'} : A}
			{refl}
\unaryRule	{z : Z \vdash \tau \equiv \tau' : \rewrite{t}{t'} : A}
			{z : Z \vdash \tau' \equiv \tau : \rewrite{t}{t'} : A}
			{symm}
\binaryRule	{z : Z \vdash \tau' \equiv \tau'' : \rewrite{t}{t'} : A}
			{z : Z \vdash \tau \equiv \tau' : \rewrite{t}{t'} : A}
			{z : Z \vdash \tau \equiv \tau'' : \rewrite{t}{t'} : A}
			{trans}
	
\binaryRule	{z : Z \vdash \tau' \equiv \sigma' : \rewrite{t'}{t''} : A}
			{z : Z \vdash \tau \equiv \sigma : \rewrite{t}{t'} : A}
			{z : Z \vdash (\tau' \vert \tau) \equiv (\sigma' \vert \sigma)  : \rewrite{t}{t''} : A}
			{}

\binaryRule	{x : A \vdash \tau \equiv \tau' : \rewrite{t}{t'} : B}
			{z : Z \vdash \sigma \equiv \sigma' : \rewrite{u}{u'} : A}
			{z : Z \vdash \horizComp{\tau}{x \mapsto \sigma} \equiv \horizComp{\tau'}{x \mapsto \sigma'} : \rewrite{\hcomp{t}{x \mapsto u}}{\hcomp{t'}{x \mapsto u'}} : B}
			{}

==> rules/bicat/constant-and-id-rewrites.tex <==
\unaryRule	{z : Z \vdash t : A}
			{z : Z \vdash \id_t : \birewrite{t}{t} : A}
			{$\id$-intro}

\unaryRule		{\big(\sigma \in \graph(A, B)(c, c')\big)}
				{x : A \vdash \sigma(x) : \rewrite{c(x)}{c'(x)} : B}
				{2-const}

==> rules/bicat/constructors-on-rewrites.tex <==
\binaryRule	{z : Z \vdash \tau' : \rewrite{t'}{t''} : A}
			{z : Z \vdash \tau : \rewrite{t}{t'} : A}
			{z : Z \vdash \tau' \vert \tau : \rewrite{t}{t''} : A}
			{vert-comp}
			
\binaryRule	{x : A \vdash \tau : \rewrite{t}{t'} : B}
			{z : Z \vdash \sigma : \rewrite{u}{u'} : A}
			{z : Z \vdash \horizComp{\tau}{x \mapsto \sigma} : \rewrite{\hcomp{t}{x \mapsto u}}{\hcomp{t'}{x \mapsto u'}} : B}
			{horiz-comp}

==> rules/bicat/contexts.tex <==
\binaryRule	{\:}
			{}
			{x : A \mathrm{\: ctx}}
			{$\big(A \in \nodes{\graph}\big)$}

==> rules/bicat/hcomp-vcomp-preservation.tex <==
\binaryRule	{x : A \vdash t : B}
			{z : Z \vdash u : A}
			{z : Z \vdash \hcomp{\id_t}{x \mapsto u} \equiv \id_{\hcomp{t}{x \mapsto u}} : \rewrite{\hcomp{t}{x \mapsto u}}{\hcomp{t}{x \mapsto u}} : B}
			{hcomp preserves $\id$}

\begin{footnotesize}
\begin{bprooftree}
\AxiomC{$x : A \vdash \tau : \rewrite{t}{t'} : B$}
\noLine
\UnaryInfC{$x : A \vdash \tau' : \rewrite{t'}{t''} : B$}
\AxiomC{$z : Z \vdash \sigma : \rewrite{u}{u'} : A$}
\noLine
\UnaryInfC{$z : Z \vdash \sigma' : \rewrite{u'}{u''} : A$}
\RightLabel{{\scriptsize interchange}}
\BinaryInfC{$z : Z \vdash \horizComp{\tau'}{x \mapsto \sigma'} \vert \horizComp{\tau}{x \mapsto \sigma} \equiv \horizComp{(\tau' \vert \tau)}{x \mapsto \sigma' \vert \sigma} : \rewrite{\hcomp{t}{x \mapsto u}}{\hcomp{t''}{x \mapsto u''}} : B$}
\end{bprooftree}
\end{footnotesize}\vspace{\treeskip}

==> rules/bicat/invertibility.tex <==
\unaryRule {x : A \vdash t : B} 
{x : A \vdash \subid{t}^{-1} \vert \subid{t} \equiv \id_t : \rewrite{t}{t} : B} 
{} 

\unaryRule {x : A \vdash t : B} 
{x : A \vdash \subid{t} \vert \subid{t}^{-1} \equiv \id_{\hcomp{t}{x \mapsto x}} : \rewrite{\hcomp{t}{x \mapsto x}}{\hcomp{t}{x \mapsto x}} : B} 
{} 

\begin{prooftree} 
\AxiomC{$x : X \vdash u : A$} 
\RightLabel{} 
\UnaryInfC{$x : X \vdash \proj{u}^{-1} \vert \proj{u} \equiv \id_{\hcomp{x}{x \mapsto u}} : \birewrite{\hcomp{x}{x \mapsto u}}{\hcomp{x}{x \mapsto u}} : A$} 
\end{prooftree}\vspace{\treeskip} 

\begin{prooftree} 
\AxiomC{$x : X \vdash u : A$} 
\RightLabel{} 
\UnaryInfC{$x : X \vdash \proj{u} \vert \proj{u}^{-1} \equiv \id_u : \birewrite{u}{u} : A$} 
\end{prooftree}\vspace{\treeskip} 

{\small 
\begin{prooftree} 
\alwaysNoLine 
\AxiomC{$z : Z \vdash u : A$} 
\AxiomC{$x : A \vdash v : B$} 
\AxiomC{$y : B \vdash t : C$} 
\alwaysSingleLine 
\RightLabel{} 
\TrinaryInfC{$z : Z \vdash \assoc{t, v, u}^{-1} \vert \assoc{t,v,u} \equiv \id_{\hcomp{\hcomp{t}{y \mapsto v}}{x \mapsto u}} : \rewrite{\hcomp{\hcomp{t}{y \mapsto v}}{x \mapsto u}}{\hcomp{\hcomp{t}{y \mapsto v}}{x \mapsto u}} : C$} 
\end{prooftree} 
}\vspace{\treeskip} 


{\small 
\begin{prooftree} 
\alwaysNoLine 
\AxiomC{$z : Z \vdash u : A$} 
\AxiomC{$x : A \vdash v : B$} 
\AxiomC{$y : B \vdash t : C$} 
\alwaysSingleLine 
\RightLabel{} 
\TrinaryInfC{$z : Z \vdash \assoc{t, v, u} \vert \assoc{t,v,u}^{-1} \equiv \id_{\hcomp{t}{y \mapsto \hcomp{v}{x \mapsto u}}} : \rewrite{\hcomp{t}{y \mapsto \hcomp{v}{x \mapsto u}}}{\hcomp{t}{y \mapsto \hcomp{v}{x \mapsto u}}} : C$} 
\end{prooftree} 
}\vspace{\treeskip} 


==> rules/bicat/structural-rewrites.tex <==
\begin{prooftree} 
\AxiomC{$ x : A \vdash t : B$} 
\RightLabel{\scriptsize $\subid{}$-intro} 
\UnaryInfC{$x : A \vdash \subid{t} : \birewrite{t}{\hcomp{t}{x \mapsto x}} : B$} 
\noLine 
\UnaryInfC{$x : A \vdash \subid{t}^{-1} : \birewrite{\hcomp{t}{x \mapsto x}}{t} : B$} 
\end{prooftree}\vspace{\treeskip} 

\begin{prooftree} 
\AxiomC{$x : A \vdash u : B$} 
\RightLabel{\scriptsize $\proj{}$-intro} 
\UnaryInfC{$x : A \vdash \proj{u} : \birewrite{\hcomp{x}{x \mapsto u}}{u} : B$} 
\noLine 
\UnaryInfC{$x : A \vdash \proj{u}^{-1} : \birewrite{u}{\hcomp{x}{x \mapsto u}} : B$} 
\end{prooftree}\vspace{\treeskip} 

\begin{prooftree} 
\alwaysNoLine 
\AxiomC{$z : Z \vdash u : A$} 
\AxiomC{$x : A \vdash v : B$} 
\AxiomC{$y : B \vdash t : C$} 
\alwaysSingleLine 
\RightLabel{\scriptsize $\assoc{}$-intro} 
\TrinaryInfC{$z : Z \vdash \assoc{t, v, u} : \rewrite{\hcomp{\hcomp{t}{y \mapsto v}}{x \mapsto u}}{\hcomp{t}{y \mapsto \hcomp{v}{x \mapsto u}}} : C$} 
\noLine 
\UnaryInfC{$z : Z \vdash \assoc{t, v, u}^{-1} : \rewrite{\hcomp{t}{y \mapsto \hcomp{v}{x \mapsto u}}}{\hcomp{\hcomp{t}{y \mapsto v}}{x \mapsto u}} : C$} 
\end{prooftree}\vspace{\treeskip} 

==> rules/bicat/terms.tex <==
\unaryRule	{\:}
			{x : A \vdash x : A}
			{var}

\unaryRule	{\big(c \in \graph(A, B)\big)}
			{x : A \vdash c(x) : B}
			{const}
			
\binaryRule	{x : A \vdash t : B}
			{z : Z \vdash u : A}
			{z : Z \vdash \hcomp{t}{x \mapsto u} : B}
			{horiz-comp}


==> rules/boring-common-rules.tex <==
\begin{figure*}[!h]

\centering
{\small

\begin{minipage}{\textwidth}
\begin{mdframed}
\centering
\input{rules/structural-rewrites-invertibility}
\caption{Invertibility of the structural rewrites}
\end{mdframed}
\end{minipage}

\begin{minipage}{\textwidth}
\begin{mdframed}
\centering
\input{rules/congruences}
\caption{Congruence laws \label{r:congruence-laws}}
\end{mdframed}
\end{minipage}
}

\begin{manyfigcap}
Equational theory for structural rewrites in $\langBiclone$, $\langCart$ and $\langCartClosed$. For $\langBicat$ these rules are restricted to \emph{unary} contexts.
\end{manyfigcap}
\end{figure*}

%\begin{figure*}[t]
%\centering
%\subrules{
%\input{rules/categorical-vert-comp}
%\caption{Categorical structure of vertical composition}}
%\subrules{
%\input{rules/interchange}
%\caption{Preservation rules}}
%\subrules{
%\input{rules/structural-rewrites-nat}
%\caption{Naturality rules on structural rewrites}}
%\subrules{
%\input{rules/biclone-laws}
%\caption{Biclone laws}}
%\subfloat{\vspace{1em}
%\centering
%The equational theory for $\langBicat$, $\langCart$ and $\langCartClosed$. For $\langBicat$ the rules are restricted to unary contexts.}
%\end{figure*}



==> rules/cart/derived-intro.tex <==
\unaryRule	{\Gamma \vdash t : A_1 \times \dots \times A_n}
{\Gamma \vdash \etaTimes{t} : \rewrite{t}{\pair{\hcomp{\pi_1}{u}, \dots, \hcomp{\pi_n}{u}}} : A_1 \times \dots \times A_n}
{$\etaTimes{}$-intro}
			
\unaryRule{\big(\Gamma \vdash \tau_i : \rewrite{t_i}{t_i'} : A_i\big)_{i= 1, \dots, n}}
{\Gamma \vdash \pair{\tau_1, \dots, \tau_n}: \rewrite{\pair{t_1, \dots, t_n}}{\pair{t_1', \dots, t_n'}} : A_1 \times \dots \times A_n}
{}

==> rules/ccc/derived-intro.tex <==
\unaryRule	{\Gamma \vdash u : \exptype{A}{B}}
			{\Gamma \vdash \etaExp{u} : \rewrite{u}{\lam{y}{\genevalterm{\wkn{u}{y}, y}}} : \exptype{A}{B}}
			{$\etaExp{}$-intro}

\unaryRule	{x_1 : A_1, \dots, x_n : A_n, y : B \vdash t : C}
			{x_1 : A_1, \dots, x_n : A_n \vdash \epsilonExpRewr{t, y \dot u} : \rewrite{\hcomp{\evalterm}{\lam{y}{t}, u}}{\hcomp{t}{x_i \mapsto x_i, z \mapsto u}} : C}
			{generalised $\epsilonExpRewr{}$-intro}
			
\unaryRule	{\Gamma, y : A \vdash \tau : \rewrite{t}{t'} :B}
			{\Gamma \vdash \lam{y}{\tau} : \rewrite{\lam{y}{t}}{\lam{y}{t'}} : \exptype{A}{B}}
			{$\lambda$-abstraction on rewrites}

==> rules/ccc/strict/contexts.tex <==
\unaryRule{\faketext}{x : A \ctx}{$A \in \nodes{\graph}$}

==> rules/ccc/strict/rules.tex <==
% for changing space between floats
\setlength{\floatsep}{5pt plus 1.0pt minus 2.0pt} 

\begin{figure*}[!h]
{\small
\begin{minipage}{\textwidth}
\begin{mdframed}
\centering
\input{rules/ccc/strict/contexts}
\vspace{-\treeskip}
\caption{Rules for contexts \label{fig:strict:contexts}}
\end{mdframed}
\end{minipage}

\begin{minipage}{\textwidth}
\begin{mdframed}
\centering
%\unaryRule
%	{\faketext}
%	{x : A \vdash x : A}
%	{const}
%\unaryRule{\faketext}
%	{x : A \vdash c(x) : B}
%	{$c \in \graph(A, B)$}
%
%\unaryRule
%	{\faketext}
%	{p : \prodop_n(A_1, \dots, A_n) \vdash \pi_i(p) : A_i}
%	{$(1 \leq i \leq n)$}
%\unaryRule
%	{(x : A \vdash t_i : B_i)_{i=1, \dots, n}}
%	{x : A \vdash \pair{t_1, \dots, t_n} : \prodop_n(A_1, \dots, A_n)}
%	{tupe}
%
\unaryRule
	{\faketext}
	{p : (\expobj{A}{B}) \times A \vdash \evalterm(p) : B}
	{eval}
\quad
\binaryRule
	{p : \prodop_{2}(A, B) \vdash t : C}
	{q \text{ fresh }}
	{q : A \vdash \altlam{q}{p}{t} : \exptype{B}{C}}
	{lam}
\vspace{-\treeskip}
\caption{Rules for terms \label{r:ccc:strict:terms}}
\end{mdframed}
\end{minipage}

%\begin{minipage}{\textwidth}
%\begin{mdframed}
%\centering
%\unaryRule{\faketext}
%	{x : A \vdash \constrewr : 
%		\rewrite{c(x)}{c'(x)} : B}
%	{$\constrewr \in \graph(A, B)(c,c')$}
%\vspace{-\treeskip}
%\caption{Rules for constants}
%\end{mdframed}
%\end{minipage}

\begin{minipage}{\textwidth}
\begin{mdframed}
\centering
\unaryRule{p : \prodop_2(A, B) \vdash t : C}{p : \prodop_2(A, B) \vdash \epsilonExpRewr{t} : \rewrite{\heval{\prod_2(\altlam{x}{p}{t}, B)}}{t} : C}{$\epsilonExpRewr{}$-intro}

\begin{bprooftree} 
\AxiomC{$p : \prodop_2(A, B) \vdash t : C$ \:\quad\: $x : A \vdash u : \exptype{B}{C}$} 
\noLine 
\UnaryInfC{$p : \prodop_2(A, B) \vdash \alpha : \rewrite{\heval{\prod_2(u, B)}}{t} : C$} 
\RightLabel{{\scriptsize $\transExp{\alpha}$-intro}} 
\UnaryInfC{$q : A \vdash \transExp{q, p \bind \alpha} : 
\rewrite{u}{\altlam{q}{p}{t}} : \exptype{B}{C}$} 
\end{bprooftree}  \vspace{\treeskip}

\caption{Rewrites for cartesian closed structure \label{r:ccc:strict:rewrites}}
\end{mdframed}
\end{minipage}

\begin{minipage}{\textwidth}
\begin{mdframed}
\centering

\begin{bprooftree}
\AxiomC{$p : \prodop_2(A, B) \vdash \alpha : \rewrite{\heval{\prod_2(u, B)}}{t} : C$}
\RightLabel{\scriptsize U1}
\UnaryInfC{$p : \prodop_2(A, B) \vdash \alpha \equiv \epsilonExpRewr{t} \vert 
\genevalterm{\prod_2(\transExp{p, p \bind \alpha}, B)} : 
\rewrite{\heval{\prod_2(u, B)}}{t} : C$}
\end{bprooftree}\vspace{\treeskip}

\begin{bprooftree}
\AxiomC{$x : A \vdash \gamma : \rewrite{u}{\altlam{x}{p}{t}} : \exptype{B}{C}$}
\RightLabel{\scriptsize U2}
\UnaryInfC{$x : A \vdash \gamma \equiv \transExp{p \bind \epsilonExpRewr{t} \vert \heval{\prod_2(\gamma, B)}} : \rewrite{u}{\altlam{x}{p}{t}} : \exptype{B}{C} $}
\end{bprooftree}\vspace{\treeskip}

\unaryRule	{p : \prodop_2(A, B) \vdash \alpha \equiv \alpha' : \rewrite{\heval{\prod_2(u, B)}}{t} : B}		
			{x : A \vdash 
				\transExp{x, p \bind \alpha} \equiv 
				\transExp{x, p \bind \alpha'} : 
				\rewrite{u}{\lam{x}{t}} : 
				\exptype{B}{C}}
			{cong} 

\caption{Universal property and congruence laws for  $\transExp{\alpha}$\label{r:ccc:strict:umpTrans}}
\end{mdframed}
\end{minipage}

\begin{minipage}{\textwidth}
\begin{mdframed}
\centering

\unaryRule	{x : A \vdash u : \exptype{B}{C}}
			{x : A \vdash \etaExp{u}^{-1} : \rewrite{\altlam{x}{p}{\heval{\prod_2(u, B)}}}{u} : \exptype{B}{C}}
			{$\etaExp{}^{-1}$-intro}
\begin{bprooftree} 
\AxiomC{$p : \prodop_2(A, B) \vdash t : B$} 
\RightLabel{\scriptsize $\epsilonExpRewr{}^{-1}$-intro} 
\UnaryInfC{$p : \prodop_2(A, B) \vdash \epsilonExpRewr{t}^{-1} : \rewrite{t}{\heval{\prod_2(\altlam{p}{p}{t}}} : B$} 
\end{bprooftree}\vspace{\treeskip} 

{\footnotesize
\unaryRule	{x : A \vdash u : \exptype{B}{C}}
			{x : A \vdash \etaExp{u} \vert \etaExp{u}^{-1} \equiv \id_{\altlam{x}{x}{\heval{\prod_2(u, B)}}} : \rewrite{\altlam{x}{x}{\heval{\prod_2(u, B)}}}{\altlam{x}{x}{\heval{\prod_2(u, B)}}} : \exptype{B}{C}}
			{}
}

\begin{bprooftree} 
\AxiomC{$x : A \vdash u : \exptype{B}{C}$} 
\UnaryInfC{$x : A \vdash \etaExp{u}^{-1} \vert \etaExp{u} \equiv \id_{u} : \rewrite{u}{u} : \exptype{B}{C}$} 
\end{bprooftree}
\qquad
\begin{bprooftree} 
\AxiomC{$p : \prodop_2(A, B) \vdash t : B$} 
\UnaryInfC{$p : \prodop_2(A, B) \vdash \epsilonExpRewr{t} \vert \epsilonExpRewr{t}^{-1} \equiv \id_t  : \rewrite{t}{t} : B$} 
\end{bprooftree}

\small
\begin{prooftree} 
\AxiomC{$p : \prodop_2(A, B) \vdash t : C$} 
\UnaryInfC{$p : \prodop_2(A, B) \vdash \epsilonExpRewr{t}^{-1} \vert \epsilonExpRewr{t} \equiv \id_{\heval{\prod_2(\altlam{p}{p}{t}}} : \rewrite{\heval{\prod_2(\altlam{p}{p}{t}}}{\heval{\prod_2(\altlam{p}{p}{t}}} : C$} 
\end{prooftree}\vspace{0.5\treeskip} 
\normalsize

\caption{Invertibility rules\label{r:ccc:strict:invertibility}}
\end{mdframed}
\end{minipage}
}

\begin{manyfigcap}
Rules for $\langCom(\sig)$, for 
a \emph{unary} $\langCartClosed$-signature 
$\sig = (\baseTypes, \graph)$.
\end{manyfigcap}

\end{figure*}


==> rules/hir/ccc-eq-theory.tex <==
\setlength{\floatsep}{5pt plus 1.0pt minus 2.0pt} 

\begin{figure*}[!h]
\centering

\begin{minipage}{\textwidth}
\begin{mdframed}
\centering

\unaryRule{(\Gamma \vdash t_i : A_i)_{i=1,\dots, n}}
			{\Gamma \vdash \id_{\seq{t_1, \dots, t_n}} \equiv \seq{\id_{t_1}, \dots, \id_{t_n}} : \rewrite{\seq{t_1, \dots, t_n}}{\seq{t_1, \dots, t_n}} : \prodop_n(A_1,\dots, A_n)}
			{}
			
\unaryRule{\Gamma \vdash t : \prodop_n(A_1, \dots, A_n)}
		{\Gamma \vdash \pi_k(\id_t) \equiv \id_{\pi_k(t)} : \rewrite{\pi_k(t)}{\pi_k(t)} : A_k}
		{$(1 \leq k \leq n)$}
		
\binaryRule{\Gamma \vdash t : \exptype{A}{B}}{\Gamma \vdash u : A}{\Gamma \vdash \app{\id_t}{\id_u} \equiv \id_{\app{t}{u}} : \rewrite{\app{t}{u}}{\app{t}{u}} : B}{}
\unaryRule{\Gamma, x : A \vdash t : B}{\Gamma \vdash \lam{x}{\id_t} \equiv \id_{\lam{x}{t}} : \rewrite{\lam{x}{t}}{\lam{x}{t}} : \exptype{A}{B}}{} \vspace{-\treeskip}

\binaryRule{(\Gamma \vdash \tau'_i : \rewrite{t_i'}{t_i''} : A_i)_{i=1,\dots, n}}
			{(\Gamma \vdash \tau_i : \rewrite{t_i}{t_i'} : A_i)_{i=1,\dots, n}}
			{\Gamma \vdash \seq{\ind{\tau}' \vert \ind{\tau}} \equiv \seq{\ind{\tau}'} \vert \seq{\ind{\tau}} : \rewrite{\seq{t_1, \dots, t_n}}{\seq{t_1'', \dots, t_n''}} : \prodop_n(A_1, \dots, A_n)}
			{}

\binaryRule{\Gamma \vdash \tau' : \rewrite{t'}{t'} : \prodop_n(A_1, \dots, A_n)}{\Gamma \vdash \tau : \rewrite{t}{t'} : \prodop_n(A_1, \dots, A_n)}{\Gamma \vdash \pi_k(\tau' \vert \tau)\equiv \pi_k(\tau') \vert \pi_k(\tau) : \rewrite{\pi_k(t)}{\pi_k(t'')} : A_k}{$(1 \leq k \leq n)$}

\begin{bprooftree}
\AxiomC{$\Gamma \vdash \tau' : \rewrite{t'}{t''} : \exptype{A}{B}$}
\noLine
\UnaryInfC{$\Gamma \vdash \tau : \rewrite{t}{t'} : \exptype{A}{B}$}
\AxiomC{$\Gamma \vdash \sigma' : \rewrite{u'}{u''} : A$}
\noLine
\UnaryInfC{$\Gamma \vdash \sigma : \rewrite{u}{u'} : A$}
\BinaryInfC{$\Gamma \vdash (\app{\tau'}{\sigma'}) \vert (\app{\tau}{\sigma}) \equiv \app{(\tau' \vert \tau)}{(\sigma' \vert \sigma)} : \rewrite{\app{t}{u}}{\app{t''}{u''}} : B$}
\end{bprooftree} \vspace{\treeskip} 

\binaryRule{\Gamma, x: A \vdash \tau' : \rewrite{t'}{t''} : B}{\Gamma, x: A \vdash \tau : \rewrite{t}{t'} : B}{\Gamma \vdash \lam{x}{(\tau' \vert \tau)} \equiv \lam{x}{\tau'} \vert \lam{x}{\tau} : \rewrite{\lam{x}{t}}{\lam{x}{t''}} : \exptype{A}{B}}{}

\caption{Functoriality of the constructors \label{fig:hir:functorality}}
\end{mdframed}
\end{minipage}

\begin{minipage}{\textwidth}
\begin{mdframed}
\centering
			
\unaryRule 	{\Gamma \vdash \tau : \rewrite{t}{t'} : \prodop_n(A_1, \dots, A_n)} 
			{\Gamma \vdash \etaTimes{t'} \vert \tau \equiv \seq{\pi_1 (\tau), \dots, \pi_n(\tau)} \vert \etaTimes{t} : \rewrite{t}{\seq{\pi_1(t), \dots, \pi_n(t)}} : \prodop_n(A_1, \dots, A_n)}
			{$\etaTimes{}$-nat}

\unaryRule	{(\Gamma \vdash \tau_i : \rewrite{t_i}{t'_i} : A_i)_{i=1,\dots, n}}
			{\Gamma \vdash \tau_k \vert \epsilonTimesInd{k}{t_1, \dots, t_n} \equiv  \epsilonTimesInd{k}{t_1', \dots, t_n'} \vert \pi_k(\seq{\tau_1, \dots, \tau_n}) : \rewrite{\pi_k(\seq{t_1, \dots, t_n})}{t_k'} : A_k}
			{$\epsilonTimesInd{k}{}$-nat}

\unaryRule	{\Gamma \vdash \tau : \rewrite{t}{t'} : \exptype{A}{B}}
			{\Gamma \vdash \big(\lam{x}{(\app{\tau}{\id_x})}\big) \vert \etaExp{t} \equiv \etaExp{t'} \vert \tau : \rewrite{t}{\lam{x}{(\app{t'}{x}})} : \exptype{A}{B}}
			{$\etaExp{}$-nat}

\begin{small}
\begin{bprooftree}
\AxiomC{$\Gamma, x : A \vdash \tau : \rewrite{t}{t'} : B$}
\noLine
\UnaryInfC{$\Gamma \vdash \sigma : \rewrite{u}{u'} : A$}
\AxiomC{$\Gamma = (x_i : A_i)_{i=1,\dots, n}$}
\RightLabel{{\scriptsize $\genEpsilonExp{}$-nat}}
\BinaryInfC{$\Gamma \vdash \genEpsilonExp{x \bind t', u'} \vert \big(\app{(\lam{x}{\tau})}{\sigma}\big) \equiv \horizComp{\tau}{x_i \mapsto \id_{x_i}, x \mapsto \sigma} \vert \genEpsilonExp{x \bind t, u} : \rewrite{\app{(\lam{x}{t})}{u}}{t'[u'/x]} : B$}
\end{bprooftree}
\end{small}

\caption{\label{r:rewritesNat} Naturality laws}
\end{mdframed}
\end{minipage}

\end{figure*}

\begin{figure*}[h]

\begin{minipage}{\textwidth}
\begin{mdframed}
\centering

\unaryRule	{\Gamma \vdash t : \prodop_n(A_1, \dots, A_n)}
			{\Gamma \vdash \epsilonTimesInd{k}{\pi_1(t), \dots, \pi_n(t)} \vert \pi_k (\etaTimes{t}) \equiv \id_{\pi_k t} : \rewrite{\pi_k t}{\pi_k t} : A_k}
			{$\Delta^\times_1$, $1 \leq k \leq n$}

\unaryRule	{(\Gamma \vdash t_i : A_i)_{i=1,\dots, n}}
			{\Gamma \vdash \seq{\epsilonTimesInd{1}{t_1, \dots, t_n}, \dots, \epsilonTimesInd{n}{t_1, \dots, t_n}} \vert \etaTimes{\seq{\ind{t}}} \equiv \id_{\seq{\ind{t}}} : \rewrite{\seq{\ind{t}}}{\seq{\ind{t}}} : \prodop_n(A_1, \dots, A_n)}
			{$\Delta^\times_2$}

\unaryRule	{\Gamma, x : A \vdash t : B }
			{\Gamma \vdash \big(\lam{x}{\genEpsilonExp{x \bind t, x}}\big) \vert \etaExp{\lam{x}{t}} \equiv \id_{\lam{x}{t}}			: \lam{x}{t} \To \lam{x}{t} : \exptype{A}{B} }
			{$\Delta^\to_1$}

\binaryRule	{\Gamma \vdash t : \exptype{A}{B}}
			{x \notin \dom(\Gamma)}
			{\Gamma, y : A \vdash \genEpsilonExp{x \bind (\app{t}{x}), y} \vert (\app{\etaExp{t}}{\id_x}) \equiv \id_{\app{t}{x}}			: \app{t}{x} \To \app{t}{x} : B }
			{$\Delta^\to_2$}
\caption{\label{r:hir:triangleLaws} Triangle identities}
\end{mdframed}
\end{minipage}

\begin{minipage}{\textwidth}
\begin{mdframed}
\centering 

\input{rules/hir/invertibility-congruences}

\caption{Invertibility of the unit and counit}
\end{mdframed}
\end{minipage}

\end{figure*}

\begin{figure*}[ht]

\begin{minipage}{\textwidth}
\begin{mdframed}
\centering 

\unaryRule{(\Gamma \vdash \tau_i \equiv \tau_i' : \rewrite{t_i}{t_i'} : A_i)_{i=1, \dots, n}}
		{\Gamma \vdash \seq{\tau_1, \dots, \tau_n} \equiv \seq{\tau_1', \dots, \tau_n'} : \rewrite{\seq{t_1, \dots, t_n}}{\seq{t_1', \dots, t_n'}} : \prodop_n(A_1, \dots, A_n)}
		{}

\unaryRule{\Gamma \vdash \tau \equiv \tau' : \rewrite{t}{t'} : \prodop_n(A_1, \dots, A_n)}
		{\Gamma \vdash \pi_k(\tau) \equiv \pi_k(\tau') : \rewrite{\pi_k(t)}{\pi_k(t)} : A_k}
		{$(1 \leq k \leq n)$}
		
\binaryRule{\Gamma \vdash \tau \equiv \tau' : \rewrite{t}{t'} : \exptype{A}{B}}
			{\Gamma \vdash \sigma \equiv \sigma' : \rewrite{u}{u'} : A}
			{\Gamma \vdash (\app{\tau}{\sigma}) \equiv (\app{\tau'}{\sigma'}) : \rewrite{\app{t}{u}}{\app{t'}{u'}} : B}
			{}		
		
\unaryRule{\Gamma, x : A \vdash \tau \equiv \tau' : \rewrite{t}{t'} : B}
			{\Gamma \vdash \lam{x}{\tau} \equiv \lam{x}{\tau'} : \rewrite{\lam{x}{t}}{\lam{x}{t'}} : \exptype{A}{B}}
			{}

\caption{Congruence laws \label{fig:hir:congruence-laws}}
\end{mdframed}
\end{minipage}

\begin{manyfigcap}
Equational theory for $\hirCCC(\graph)$
\end{manyfigcap}

\end{figure*}

==> rules/hir/ccc-intro-rules.tex <==
\setlength{\floatsep}{5pt plus 1.0pt minus 2.0pt} 

\begin{figure*}[!ht]
\small

\begin{minipage}{\textwidth}
\begin{mdframed}
\centering

\input{rules/hir/basic-terms}

\unaryRule{\Gamma \vdash t : \prodop_n(A_1, \dots, A_n)}
		{\Gamma \vdash \pi_k(t) : A_k}
		{proj}
\unaryRule{(\Gamma \vdash t_i : A_i)_{i=1,\dots,n}}{\Gamma \vdash \seq{t_1, \dots, t_n} : \prodop_n(A_1, \dots, A_n)}{prod}\vspace{-\treeskip}

\unaryRule{\Gamma, x : A \vdash t : B}{\Gamma \vdash \lam{x}{t} : \exptype{A}{B}}{lam}
\binaryRule{\Gamma \vdash t : \exptype{A}{B}}{\Gamma \vdash u: A}{\Gamma \vdash \app{t}{u} : B}{app} 
\caption{\label{fig:r:strict-ccc:terms} Rules for terms in $\hirCCC(\graph)$}
\end{mdframed}
\end{minipage}

\begin{minipage}{\textwidth}
\begin{mdframed}
\centering

\input{rules/hir/basic-rewrites}

\begin{bprooftree}
\AxiomC{$\Gamma \vdash t : \prodop_n(A_1, \dots, A_n)$}
\RightLabel{\scriptsize $\etaTimes{}$-intro}
\UnaryInfC{$\Gamma \vdash \etaTimes{t} : \rewrite{t}{\seq{\pi_1(t), \dots,\pi_n(t)} : \prodop_n(A_1, \dots, A_n)}$}
\noLine
\UnaryInfC{$\Gamma \vdash \etaTimes{t}^{-1} : \rewrite{\seq{\pi_1(t), \dots,\pi_n(t)}}{t} : \prodop_n(A_1, \dots, A_n)$}
\end{bprooftree} \vspace{\treeskip}

\begin{bprooftree}
\AxiomC{$\Gamma \vdash \seq{t_1, \dots, t_n} : \prodop_n(A_1, \dots, A_n)$}
\RightLabel{\scriptsize $\epsilonTimesInd{k}{}$-intro $(1 \leq k \leq n)$}
\UnaryInfC{$\Gamma \vdash \epsilonTimesInd{k}{t_1, \dots, t_n} : \rewrite{\pi_k(\seq{t_1, \dots, t_n})}{t_k} : A_k$}
\noLine
\UnaryInfC{$\Gamma \vdash \epsilonTimesInd{-k}{t_1, \dots, t_n} : \rewrite{t_k}{\pi_k(\seq{t_1, \dots, t_n})} : A_k$}
\end{bprooftree} \vspace{\treeskip}

\begin{bprooftree}
\AxiomC{$\Gamma \vdash t : \exptype{A}{B}$}
\RightLabel{\scriptsize $\etaExp{}$-intro}
\UnaryInfC{$\Gamma \vdash \etaExp{t} : \rewrite{t}{\lam{x}{(\app{t}{x})}} : \exptype{A}{B}$}
\noLine
\UnaryInfC{$\Gamma \vdash \etaExp{t}^{-1} : \rewrite{\lam{x}{(\app{t}{x})}}{t} : \exptype{A}{B}$}
\end{bprooftree}
\begin{bprooftree}
\AxiomC{$\Gamma, x : A \vdash t : B$}
\AxiomC{$\Gamma \vdash u : A$}
\RightLabel{\scriptsize $\beta$-intro}
\BinaryInfC{$\Gamma \vdash \genEpsilonExp{x \bind t, u} : \rewrite{\app{(\lam{x}{t})}{u}}{t[u/x]} : B$}
\noLine
\UnaryInfC{$\Gamma \vdash \genEpsilonExp{x \bind t, u}^{-1} : \rewrite{t[u/x]}{\app{(\lam{x}{t})}{u}} : B$}
\end{bprooftree}\vspace{\treeskip}

\unaryRule{(\Gamma \vdash \tau_i : \rewrite{t_i}{t_i'} : A_i)_{i=1,\dots,n}}{\Gamma \vdash \seq{\tau_1, \dots, \tau_n} : \rewrite{t_1, \dots, t_n}{t_1', \dots, t_n'} : \prodop_n(A_1, \dots, A_n)}{2-prod}

\unaryRule{\Gamma \vdash \tau : \rewrite{t}{t'} : \prodop_n(A_1, \dots, A_n)}{\Gamma \vdash \pi_k(\tau) : \rewrite{\pi_k(t)}{\pi_k(t')} : A_k}{2-proj $(1 \leq k \leq n)$}

\unaryRule{\Gamma, x : A \vdash \tau : \rewrite{t}{t'} : B}{\Gamma \vdash \lam{x}{\tau} : \rewrite{\lam{x}{t}}{\lam{x}{t'}} : \exptype{A}{B}}{2-lam}

\binaryRule{\Gamma \vdash \tau : \rewrite{t}{t'} : \exptype{A}{B}}{\Gamma \vdash \sigma : \rewrite{u}{u'} : A}{\Gamma \vdash \app{\tau}{\sigma} : \rewrite{\app{t}{u}}{\app{t'}{u'}} : B}{2-app}

\caption{\label{fig:r:strict-ccc:rewrites} Rules for rewrites in $\hirCCC(\graph)$}
\end{mdframed}
\end{minipage}

\end{figure*}

==> rules/hir/invertibility-congruences.tex <==
\begin{small}
\unaryRule	{\Gamma \vdash t_1 : A_1 \qquad \dots \qquad \Gamma \vdash t_n : A_n}
			{\Gamma \vdash \epsilonTimesInd{-k}{t_1, \dots, t_n} \vert \epsilonTimesInd{k}{t_1, \dots, t_n} \equiv \id_{\hcomp{\pi_k}{\seq{t_1, \dots, t_n}}}  : \rewrite{\hcomp{\pi_k}{\seq{t_1, \dots, t_n}}}{\hcomp{\pi_k}{\seq{t_1, \dots, t_n}}} : A_k} 
			{$(1 \leq k \leq n)$}
\end{small}

\unaryRule	{\Gamma \vdash t_1 : A_1 \qquad \dots \qquad \Gamma \vdash t_n : A_n}
			{\Gamma \vdash \epsilonTimesInd{k}{t_1, \dots, t_n} \vert \epsilonTimesInd{-k}{t_1, \dots, t_n} \equiv \id_{t_k} : \rewrite{t_k}{t_k} : A_k} 
			{$(1 \leq k \leq n)$}		
						
\unaryRule	{\Gamma \vdash t : \prodop_n(A_1, \dots, A_n)}
			{\Gamma \vdash \etaTimes{t}^{-1} \vert \etaTimes{t} \equiv \id_{t} : \rewrite{t}{t} : \prodop_n(A_1, \dots, A_n)}
			{}

\unaryRule	{\Gamma \vdash t : \prodop_n(A_1, \dots, A_n)}
			{\Gamma \vdash \etaTimes{t} \vert \etaTimes{t}^{-1}  \equiv \id_{\seq{\hcomp{\pi_1}{t}, \dots, \hcomp{\pi_n}{t}}} : \rewrite{\seq{\hcomp{\ind{\pi}}{t}}}{\seq{\hcomp{\ind{\pi}}{t}}} : \prodop_n(A_1, \dots, A_n)}
			{}

{\small
\unaryRule	{\Gamma \vdash u : \exptype{A}{B}}
			{\Gamma \vdash \etaExp{u} \vert \etaExp{u}^{-1} \equiv \id_{\lam{x}{(\app{u}{x})}} : \rewrite{\lam{x}{(\app{u}{x})}}{\lam{x}{(\app{u}{x})}} : \exptype{A}{B}}
			{}
}

\begin{bprooftree} 
\AxiomC{$\Gamma \vdash u : \exptype{A}{B}$} 
\UnaryInfC{$\Gamma \vdash \etaExp{u}^{-1} \vert \etaExp{u} \equiv \id_{u} : \rewrite{u}{u} : \exptype{A}{B}$} 
\end{bprooftree} \vspace{\treeskip}

\begin{bprooftree} 
\AxiomC{$\Gamma, x : A \vdash t : B$} 
\AxiomC{$\Gamma \vdash u : A$}
\BinaryInfC{$\Gamma \vdash \genEpsilonExp{x \bind t, u} \vert \genEpsilonExp{x \bind t, u}^{-1} \equiv \id_{t[u/x]}  : \rewrite{t[u/x]}{t[u/x]} : B$} 
\end{bprooftree}
\vspace{\treeskip} 

\begin{small}
\begin{prooftree} 
\AxiomC{$\Gamma, x : A \vdash t : B$} 
\AxiomC{$\Gamma \vdash u : A$}
\BinaryInfC{$\Gamma \vdash \genEpsilonExp{x \bind t, u}^{-1} \vert \genEpsilonExp{x \bind t, u} \equiv \id_{\app{(\lam{x}{t})}{u}} : \rewrite{\app{(\lam{x}{t})}{u}}{\app{(\lam{x}{t})}{u}} : B$} 
\end{prooftree}
\end{small}
